Random Number Generator, Zero-Crossing, and Nonlinearity Attacks against the Kirchhoff-Law-Johnson-Noise (KLJN) Secure Key Exchange Protocol

This dissertation demonstrates three new types of attacks against the KLJN scheme. The first attack type is based on compromised RNGs. The first RNG attacks are deterministic. First, Eve knows both noises. She can crack the bit via Ohm's Law and one-bit powers within a fraction of the bit exchange period. Second, Eve knows only Bob's noise, so she can learn Bob's resistance value via Ohm's Law and Alice's resistance at the end of the bit exchange period. She can also use a process of elimination. The second RNG attacks are statistical. First, Eve has partial knowledge of Alice's and Bob's noises. She can crack the bit by taking the highest cross-correlation between her noises and the measured noise in the wire, and by taking the highest cross-correlation between her noises and Alice's/Bob's noises. Second, Eve has partial knowledge of only Alice's noise. She can still crack the bit, but after the bit exchange period. The second attack type is based on thermodynamics. Previously, the KLJN scheme required thermal equilibrium. However, Vadai, et al, in (Nature) Science Reports shows a modified scheme, where there is a non-zero thermal noise, yet the system resists all the known attacks. We utilize coincidence events between the line current and voltage and show that there is non-zero information leak. As soon as thermal equilibrium is restored, the system is perfectly secure again. The final attack type is based on the nonlinearity of the noise generators. We explore the effect of distortion at the second and third orders. It is demonstrated that 1% distortion results in a significant information leak. We also show that decreasing the effective temperature results in the KLJN scheme approaching perfect security.

==> data/RNG_complete.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Fall 2016.  
%
%
%  Author: Sean Zachary Roberson
%  Version 3.17.09
%  Last Updated: 9/21/2017
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                           SECTION I
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\chapter{\uppercase {Random Number Generator Attack against the Kirchhoff-Law-Johnson-Noise Secure Key Exchanger}\textsuperscript{1,2}}\label{RNG_chapter}
\blfootnote{\textsuperscript{1}Part of this chapter is reprinted with permission from C.~Chamon, S.~Ferdous, and L.~B.~Kish, ``Deterministic random number generator attack against the Kirchhoff-law-Johnson-noise secure key exchange protocol," {\it Fluctuation and Noise Letters}, vol. 20, no. 5, 2021. Copyright 2021 by World Scientific Publishing Company.}
\blfootnote{\textsuperscript{2}Part of this chapter is reprinted with permission from C.~Chamon, S.~Ferdous, and L.~B.~Kish, ``Statistical random number generator attack against the Kirchhoff-law-Johnson-noise secure key exchange protocol," {\it Fluctuation and Noise Letters}, accepted for publication, 2021. Copyright 2021 by World Scientific Publishing Company.}
\section{Random Number Generator Attacks}
\label{RNG}

There are two classes of practical random number generators: true (physical) and computational. The nature of computational RNGs is that they collect randomness from various low-entropy input streams and try to generate outputs that are in practice indistinguishable from truly random streams \cite{RNG1,RNG2,RNG3,RNG4,RNG5,RNG6}. The randomness of an RNG relies on the uncertainty of the random seed, or initialization vector, and a long sequence with uniform distribution. The moment an adversary learns the seed, the outputs are known, and the RNG is compromised.

Various RNG attacks exist against conditionally secure communications \cite{RNG1,RNG2,RNG3,RNG4,RNG5,RNG6}. Unconditionally secure communications also require true random numbers for perfect security. That is also true for the noises of Alice and Bob, and for the randomness of their switch driving. Yet, it is unclear how Eve can utilize compromised RNGs to attack the KLJN scheme. Here, we demonstrate with simple attack examples that compromised noises lead to information leak. 

The rest of this chapter is organized as follows. Section~\ref{detRNGexperiment} describes the new deterministic attack protocols, Section~\ref{detRNGresults} demonstrates their results, and Section~\ref{detRNGtransition} closes this part of the chapter. Then, Section~\ref{statRNGattack} describes the new statistical attack protocols, Section~\ref{statRNGresults} demonstrates their results, and Section~\ref{statRNGtransition} closes this chapter.

\section{Deterministic RNG Attack against the KLJN Scheme}
\label{detRNG_entire}

\subsection{Attack Methodology}
\label{detRNGexperiment}

Two theoretical situations are introduced where Eve can use compromised RNGs to crack the KLJN scheme: one where Eve knows the roots of both Alice’s and Bob’s generators (bilateral parameter knowledge), and another where Eve knows the root of only Bob's generator (unilateral parameter knowledge). A scenario is also introduced where the only statistical evaluation needed is in the rarely-occurring event of a negligible waiting/verification (no-response) time.

\subsubsection{Bilateral Parameter Knowledge}
\label{bilateral}
\paragraph{\it Ohm's Law}\mbox{}\\
Eve knows the roots of both Alice’s and Bob’s RNGs, thus she knows the instantaneous amplitudes of the noise voltage generators for each of their resistors (see Figure~\ref{figKLJN}). With $U_{\mathrm{H,A}}(t)$, $U_{\mathrm{L,A}}(t)$, $U_{\mathrm{H,B}}(t)$, and $U_{\mathrm{L,B}}(t)$ known, Eve measures the wire voltage $U_{\mathrm{w}}(t)$ and the wire current  $I_{\mathrm{w}}(t)$ to determine $R_{\mathrm{B}}$ (see Equation~\eqref{Uw}) and determines that the correct waveform for $R_{\mathrm{B}}$ is a flat line at the expected resistor value, while the incorrect waveform is a noise with divergent spikes. This is because the difference between $U_{\mathrm{w}}(t)$ and $U_{\mathrm{B}}(t)$ is directly proportional to $I_{\mathrm{w}}(t)$, with $R_{\mathrm{B}}$ as the scaling factor, and the incorrect noise voltage for $U_{\mathrm{B}}(t)$ would not render a constant value for $R_{\mathrm{B}}$.

A realization of the waveforms for $R_{\mathrm{B}}$ is shown in Figure~\ref{RB} at $R_{\mathrm{H}} = 100$~k\textOmega, $R_{\mathrm{L}} = 10$~k\textOmega, $T_{\mathrm{eff}} = 10^{18}$~K, and $\Delta f_{\mathrm{B}} = 500$~Hz. At the present situation, the flat line corresponds to $R_{\mathrm{H}}$, thus Eve determines that Bob has chosen $R_{\mathrm{H}}$. With $U_{\mathrm{A}}(t)$, $U_{\mathrm{B}}(t)$, $R_{\mathrm{B}}$, and $I_{\mathrm{w}}(t)$ known, Eve uses Equation~\eqref{Iw} to solve for $R_{\mathrm{A}}$.

\begin{figure}[ht!]
\centering
	\includegraphics[width=6in]{resistor_waveform.pdf}
\caption{\ A realization of the waveforms for $R_{\mathrm{B}}$ (see Equation~\eqref{Uw}) at $R_{\mathrm{H}} = 100$~k\textOmega, $R_{\mathrm{L}} = 10$~k\textOmega, $T_{\mathrm{eff}} = 10^{18}$~K, and $\Delta f_{\mathrm{B}} = 500$~Hz. The flat line corresponds to $R_{\mathrm{H}}$, thus Eve determines that Bob has chosen $R_{\mathrm{H}}$. The incorrect waveform is a noise with divergent spikes.}
\label{RB}
\end{figure}

\paragraph{\it One-Bit Powers}\mbox{}\\
Eve knows the roots of both Alice’s and Bob’s RNGs, thus she knows the instantaneous amplitudes of the noise voltage generators for each of their resistors (see Figure~\ref{figKLJN}). With $U_{\mathrm{H,A}}(t)$, $U_{\mathrm{L,A}}(t)$, $U_{\mathrm{H,B}}(t)$, and $U_{\mathrm{L,B}}(t)$ known, Eve uses Equations~\eqref{Uw} and \eqref{Iw} to come up with the four possible waveforms for $U_{\mathrm{w}}(t)$ and $I_{\mathrm{w}}(t)$ and therefore the four possible waveforms for the instantaneous power flow from Alice to Bob, given by

\begin{equation}
P_\mathrm{w}(t)=U_\mathrm{w}(t)I_\mathrm{w}(t).\label{Pw}
\end{equation}

\noindent Eve measures $U_{\mathrm{w}}(t)$ and $I_{\mathrm{w}}(t)$ and determines the actual $P_{\mathrm{w}}(t)$, which will be identical to one of her four hypothetical waveforms.

Note, the protocol shown above can be simplified to the extreme: Eve's instruments may have just one bit resolution, which is suitable to determine solely the instantaneous direction of the power flow.

\subsubsection{Unilateral Parameter Knowledge}
\label{unilateral}
\paragraph{\it Ohm's Law}\mbox{}\\
Eve knows only the root of Bob's generator RNG, thus she knows merely the noise generator outputs of Bob's resistors, $U_{\mathrm{L,B}}(t)$ and $U_{\mathrm{H,B}}(t)$. Alice's generator voltages are unknown to her. Eve uses the same protocol as mentioned in the bilateral case (see Section~\ref{bilateral}) to determine $R_{\mathrm{B}}$, but because Alice’s generator voltages are unknown to her, she cannot use Equation~\eqref{Iw} to solve for $R_{\mathrm{A}}$. Instead, she uses the KLJN protocol as Bob does: use the entire bit exchange period to evaluate the measured mean-squared voltage on the wire. From that value, by using Equation~\eqref{meansquare}, she evaluates the parallel resultant $R_{\mathrm{P}}$ of the resistances of Alice and Bob. From $R_{\mathrm{P}}$ and $R_{\mathrm{B}}$, she can calculate $R_{\mathrm{A}}$. This method can still be applied in case Eve is not sure of her result from the bilateral case (see Section~\ref{bilateral}).

\paragraph{\it Process of Elimination}\mbox{}\\
Eve knows the root of Alice’s RNG. Thus, she knows merely the noise generator outputs of Alice’s resistors, $U_{\mathrm{L,A}}(t)$ and $U_{\mathrm{H,A}}(t)$. Bob’s generator voltages are unknown to her. Eve measures the wire voltage $U_{\mathrm{w}}(t)$ and wire current $I_{\mathrm{w}}(t)$. Then, she calculates the hypothetical voltage drops on Alice's possible choice of resistances $R_{\mathrm{H}}$ and $R_{\mathrm{L}}$. With these data, she tests two hypotheses:

\noindent\begin{description}%[leftmargin=!,labelwidth=\widthof{The longest label}]
\item [Hypothesis (i):] Alice has chosen $R_{\textrm{L}}$.
\item [Hypothesis (ii):] Alice has chosen $R_{\textrm{H}}$.
\end{description}

With Hypothesis (i), Eve takes the sum

\begin{equation}
U^\ast_{\mathrm{R_L}}(t)=U_{\mathrm{w}}(t)+I_{\mathrm{w}}(t)R_{\mathrm{L}}.\label{UA}
\end{equation}

\noindent To test Hypothesis (i) she compares the $U_{\mathrm{A}}(t)$ determined by Equation~\eqref{UA} to $U_{\mathrm{L,A}}(t)$. If they are identical, then Hypothesis (i) is correct, otherwise Hypothesis (ii) is valid.

Finally, Eve evaluates the measured mean-square voltage on the wire over the bit exchange period. From that value, by using Equation~\eqref{meansquare}, she evaluates the parallel resultant $R_{\mathrm{P}}$ of the resistances of Alice and Bob. From $R_{\mathrm{P}}$ and $R_{\mathrm{A}}$, she calculates $R_{\mathrm{B}}$, thus she has cracked the KLJN scheme.

\subsubsection{Timing}
\label{timing}
In each attack, Eve may or may not know which noise belongs to which resistor, or the noises may provide a voltage-to-current ratio that results in either $R_{\mathrm{H}}$ or $R_{\mathrm{L}}$. In these scenarios, there will be a negligible waiting/verification (no-response) time before Eve can differentiate between the noises. The probability of the two independent noises being equal at any given point is

\begin{equation}
p_{\mathrm{0}}=\frac{1}{2^\Delta},\label{p0}
\end{equation}

\noindent where $\Delta$ is the number of resolution bits.

We can consider the event that the noises run identically for $n$ subsequent steps to be a geometric distribution, with a probability of

\begin{equation}
p=p_0^n,\label{p1}
\end{equation}

\noindent where $n=t/\tau$ and $\tau$ is the autocorrelation time, given by the Nyquist Sampling Theorem

\begin{equation}
\tau\approx\frac{1}{2\Delta f_{\mathrm{B}}}.\label{tau}
\end{equation}

\noindent The approximation sign is due to the quantized nature of the noises, as they are constant throughout the bit exchange periods.

While such an identical match between the two noises is taking place, Eve cannot distinguish between the two noises, thus the actual resistance situation (see Figure~\ref{threelevels}) remains secure. However, the exponential decay in Equation~\eqref{p1} yields an efficient cracking scheme of the secure key bit value within a short amount of time. In accordance with Equation~\eqref{p1}, the probability of the two independent seeds running identically is

\begin{equation}
p\approx p_0^{t/\tau}\approx\left(\frac{1}{2^\Delta}\right)^{t/\tau}.\label{p}
\end{equation}

\subsection{Demonstration}
\label{detRNGresults}
\subsubsection{Johnson Noise Emulation}
\label{OGnoisegen}
First, we generated Gaussian band-limited white noise (GBLWN). Precautions were used to avoid aliasing errors, improve Gaussianity, and reduce bias:

\begin{enumerate}[label=(\roman*)]
\item At first, using the MATLAB randn() function, 2\textsuperscript{24} or 16,777,216 Gaussian random numbers were generated.

\item This process was repeated 10 times to generate 10 independent raw noise series, and then an ensemble average was taken out of those 10 series to create one single noise time function with improved Gaussianity and decreased short-term bias.

\item Then this time series was converted to the frequency domain by Fast Fourier Transformation (FFT). To get rid of any aliasing error, we opened the real and imaginary portions of the FFT spectrum and doubled their frequency bandwidths by zero padding.

\item Finally, we performed an inverse FFT (IFFT) of the zero-padded spectrum to get the time function of the anti-aliased noise.
\end{enumerate}

\noindent The real portion of the IFFT result is the band-limited, anti-aliased noise with improved Gaussianity and decreased bias.

The histogram and probability plot for the generated noise are shown in Figures~\ref{hist_noise} and \ref{probplot_noise}, respectively, showing that the noise is Gaussian. Figure~\ref{PSD_noise} demonstrates that the noise has band-limited, white power density spectrum and it is anti-aliased.

\begin{figure}[H]
\centering
	\includegraphics[width=6in]{hist_noise.pdf}
\caption{Histogram of the noise. A mean of zero and a standard deviation of 1 indicates a standard normal distribution.\label{hist_noise}}
\end{figure}

\begin{figure}[H]
\centering
	\includegraphics[width=6in]{probplot_noise.pdf}
\caption{Normal-probability plot of the noise. A straight line indicates a pure Gaussian distribution.\label{probplot_noise}}
\end{figure}

\begin{figure}[H]
\centering
	\includegraphics[width=6in]{PSD_noise.pdf}
\caption{Power spectral density of the noise. The bandwidth of the noise is 500 Hz, see Equation~\eqref{meansquare}.\label{PSD_noise}}
\end{figure}

The final step was to scale this normalized Gaussian nosie (see Equation~\eqref{meansquare}) to the required level of Johnson noise for the given resistance, temperature, and bandwidth values ($R_\mathrm{L}$, $R_\mathrm{H}$, $T_\mathrm{eff}$, and $\Delta$$f_\mathrm{B}$, respectively). We chose $R_\mathrm{L}$=10 k$\Omega$, $R_\mathrm{H}$=100 k$\Omega$, $T_\mathrm{eff}$=10\textsuperscript{18} K,  and $\Delta$$f_\mathrm{B}$=500 Hz. A realization of the Johnson noise of $U_\mathrm{H,A}(t)$, $U_\mathrm{L,A}(t)$, $U_\mathrm{H,B}(t)$, and $U_\mathrm{L,B}(t)$, where $U_\mathrm{H,A}(t)$ is the noise voltage of Alice’s $R_\mathrm{H}$, $U_\mathrm{L,A}(t)$ is the noise voltage of Alice’s $R_\mathrm{L}$, $U_\mathrm{H,B}(t)$ is the noise voltage of Bob’s $R_\mathrm{H}$, and $U_\mathrm{L,B}(t)$ is the noise voltage of Bob’s $R_\mathrm{L}$ (see Figure~\ref{figKLJN}), over 100 milliseconds is displayed in Figure~\ref{allvoltages}. The histogram, probability plot, and power spectral density for those noise voltages are shown in Figures~\ref{hist}, \ref{probplot}, and \ref{PSD}, respectively.

\begin{figure}[H]
\centering
	\includegraphics[width=5in]{allvoltages.pdf}
\caption{A realization of $U_\mathrm{H,A}(t)$, $U_\mathrm{L,A}(t)$, $U_\mathrm{H,B}(t)$, and $U_\mathrm{L,B}(t)$ (see Figure~\ref{figKLJN}) displayed over 100 milliseconds. $U_\mathrm{H,A}(t)$ is the noise voltage of Alice’s $R_\mathrm{H}$, $U_\mathrm{L,A}(t)$ is the noise voltage of Alice’s $R_\mathrm{L}$, $U_\mathrm{H,B}(t)$ is the noise voltage of Bob’s $R_\mathrm{H}$, and $U_\mathrm{L,B}(t)$ is the noise voltage of Bob’s $R_\mathrm{L}$. Each time step is one millisecond.\label{allvoltages}}
\end{figure}

\begin{figure}[H]
\centering
	\includegraphics[width=6in]{hist.pdf}
\caption{Histogram of the Johnson noise of $U_\mathrm{H,A}(t)$, $U_\mathrm{L,A}(t)$, $U_\mathrm{H,B}(t)$, and $U_\mathrm{L,B}(t)$, where $U_\mathrm{H,A}(t)$ is the noise voltage of Alice’s $R_\mathrm{H}$, $U_\mathrm{L,A}(t)$ is the noise voltage of Alice’s $R_\mathrm{L}$, $U_\mathrm{H,B}(t)$ is the noise voltage of Bob’s $R_\mathrm{H}$, and $U_\mathrm{L,B}(t)$ is the noise voltage of Bob’s $R_\mathrm{L}$ (see Figure~\ref{figKLJN}). The blue histograms represent the occurrences of the noise voltages over time, and the yellow histograms represent the occurrences of the noise voltages sampled 1000 times at a specific time point. The green area represents the overlap between the blue and yellow histograms. The red line represents the best-fitting normal probability density function (PDF) for both histograms, serving to demonstrate that the noise voltages in all four cases (HH, LL, HL, and LH) are Gaussian and ergodic.\label{hist}}
\end{figure}

\begin{figure}[H]
\centering
	\includegraphics[width=6in]{probplot.pdf}
\caption{Normal-probability plot of the Johnson noise of $U_\mathrm{H,A}(t)$, $U_\mathrm{L,A}(t)$, $U_\mathrm{H,B}(t)$, and $U_\mathrm{L,B}(t)$. A straight line indicates a pure Gaussian distribution.\label{probplot}}
\end{figure}

\begin{figure}[H]
\centering
	\includegraphics[width=6in]{PSD.pdf}
\caption{Power spectral density of the Johnson noise of $U_\mathrm{H,A}(t)$, $U_\mathrm{L,A}(t)$, $U_\mathrm{H,B}(t)$, and $U_\mathrm{L,B}(t)$. The bandwidth of the noise is 500~Hz, see Equation~\eqref{meansquare}.\label{PSD}}
\end{figure}

From the Nyquist Sampling Theorem,

\begin{equation}
\tau=\frac{1}{2\Delta f_\mathrm{B}}\label{Nyquist}
\end{equation}

\noindent where $\tau$ represents the time step, a $\Delta$$f_\mathrm{B}$ of 500 Hz renders a time step of 10\textsuperscript{-3} seconds. Because this is ideal band-limited white noise, the Nyquist samples are statistically independent.

\subsubsection{Setup of Eve's Noises}
\label{EvenoisegenM}
To generate Eve's noises that are correlated with the noises in the KLJN system, independent "thermal" noises (see Section~\ref{OGnoisegen}) are added to the noises of Alice and Bob, and the resulting noises are normalized to have the same effective value as the original noises.

For example, the new correlated noise of Eve corresponding to Alice's thermal noise $U_{\mathrm{L,A}}(t)$ is

\begin{equation}
U_{\mathrm{EL,A}}(t)=U_{\mathrm{L,A}}(t)+MU^\ast_{\mathrm{EL,A}}(t),\label{Evenoise1}
\end{equation}

\noindent where $U_{\mathrm{EL,A}}(t)$ is the new correlated noise, $U^\ast_{\mathrm{EL,A}}(t)$ is an independently generated "thermal" noise for resistance value $R_{\mathrm{L}}$, and the $M$ coefficient controls the cross-correlation between Eve's and Alice's noises, $CCC_\mathrm{LA}$ (see Section~\ref{statCCCAB}). The direct relationship between $M$ and $CCC_\mathrm{LA}$ is demonstrated in Tables~\ref{bilat_sources_table} and \ref{unilat_sources_table}, respectively located in Sections~\ref{bilatsources_demo} and \ref{unilatsources_demo}. 

Note, $U_{\mathrm{EL,A}}(t)$ and $U^\ast_{\mathrm{EL,A}}(t)$ have the same effective value. Accordingly,

\begin{equation}
U^\ast_{\mathrm{EL,A}}(t)=x(t)\sqrt{4kT_{\mathrm{eff}}R_{\mathrm{L}}\Delta f_{\mathrm{B}}},\label{Evenoise2}
\end{equation}

\noindent where $x(t)$ represents a new noise with 1 Volt effective value.

However, the effective value of $U_{\mathrm{EL,A}}(t)$ does not satisfy the Johnson formula anymore, so in order to call it a thermal noise, it must be scaled to the proper level \cite{RNG}:

\begin{equation}
U_{\mathrm{L,A}}(t)=\frac{U_{\mathrm{EL,A}}(t)}{\sqrt{\big\langle \left[U_{\mathrm{EL,A}}(t)\right]^2\big\rangle}}\sqrt{4kT_{\mathrm{eff}}R_{\mathrm{L}}\Delta f_{\mathrm{B}}}.\label{Evenoise3}
\end{equation}

\noindent In this way, the same $M$ used for the different resistance choices of Alice and Bob results in the same cross-correlation coefficient between Eve's noises and the corresponding noises of the communicating parties. Thus, four new sets of independent additive noises have been generated using the same method as in Section~\ref{OGnoisegen}.

A realization of Eve’s noise voltages in comparison to Alice’s and Bob’s noise voltages over 100 milliseconds is displayed in Figure~\ref{bothnoisestogether}. $U_{\mathrm{H,A}}(t)$ is the noise voltage of Alice’s $R_{\mathrm{H}}$, $U_{\mathrm{L,A}}(t)$ is the noise voltage of Alice’s $R_{\mathrm{L}}$, $U_{\mathrm{H,B}}(t)$ is the noise voltage of Bob’s $R_{\mathrm{H}}$, and $U_{\mathrm{L,B}}(t)$ is the noise voltage of Bob’s $R_{\mathrm{L}}$ (see Figure~\ref{figKLJN}). Each time step is one millisecond.

\begin{figure}[H]
\centering
\subfloat[]{
	\label{regular_noises_M}
	\includegraphics[width=3.2in]{uncorr_voltages_AB.pdf} } 
\subfloat[]{
	\label{Eve_noises_M}
	\includegraphics[width=3in]{uncorr_voltages_Eve.pdf} } 
\caption{A realization of $U_{\mathrm{H,A}}(t)$, $U_{\mathrm{L,A}}(t)$, $U_{\mathrm{H,B}}(t)$, and $U_{\mathrm{L,B}}(t)$ (see Figure~\ref{figKLJN}) for Alice and Bob (a), and for Eve (b), at $M=1$, displayed over 100 milliseconds.}\label{bothnoisestogether}
\end{figure}

For the deterministic attack demonstration (see Section~\ref{detRNGresults}), we keep $M$ at 0, while in the statistical attack (see Section~\ref{statRNGresults}), we vary $M$.

\subsubsection{Attack Demonstration when Eve Knows Both Noises}
\label{det_bidem}
At the bilateral parameter knowledge (see Section~\ref{bilateral}), Figure~\ref{1beve} shows the hypothetical power flow waveforms generated by Eve (top four graphs). The single-bit plot of her measurement of the actual power flow $P_\mathrm{w}(t)$ is shown by the bottom graph. If the power is delivered from Alice to Bob, the single-bit value is +1, while in the opposite case the result is -1. The orange dashed lines in the upper plots indicate the power flow in the 1-bit resolution limit. At the present situation, Eve’s measured single-bit data are identical to the dashed lines in the LH scenario only, thus Eve decides that the LH is the secure resistance situation.

\begin{figure}[H]
\centering
	\includegraphics[width=5in]{1beve.pdf}
\caption{The hypothetical and their 1-bit limit waveforms for $P_\mathrm{w}(t)$ generated by Eve. $P_\mathrm{HH}(t)$ is the hypothetical power flow in the HH case, $P_\mathrm{LL}(t)$ is the hypothetical power flow in the LL case, $P_\mathrm{HL}(t)$ is the hypothetical power flow in the HL case, and $P_\mathrm{LH}(t)$ is the hypothetical power flow in the LH case. $P_\mathrm{w}(t)$ is the single-bit measurement of the actual power flow.\label{1beve}}
\end{figure}

However, similarly to the case of string verification with noise-based logic \cite{NBL}, two independent random bit sequences, such as two different binary sequences in Figure~\ref{1beve}, may run identically for $n$ subsequent steps with probability

\begin{equation}
p=\frac{1}{2^n}\label{probability}
\end{equation}

\noindent where the independence of the subsequent samples within a given binary sequence is also essential, and $n=t/\tau$.

While such an identical match between two of the 4 noises is taking place, Eve cannot decide which one of the hypothetical sequences is valid thus the actual resistor situation (see Figure~\ref{threelevels}) remains secure. However, the exponential decay of the probability of the duration of this phenomenon in Equation~\eqref{probability} yields an efficient cracking of the secure key bit value within a short time. In accordance with \eqref{probability}, the probability of two independent ones of our binary sequences (Figure~\ref{1beve}) running identically is

\begin{equation}
p(t)\approx\frac{1}{2^{t/\tau}}=\frac{1}{2^{1000t}}\label{poft}
\end{equation}

\noindent The approximation sign is due to the quantized nature of $p(t)$ because it is staying constant during the bit exchange periods.

This simulation was run 1000 times. Figure~\ref{log_securecases} shows the probability that the exchange of the current key bit is still secure. Figure~\ref{log_crack} shows the probability that Eve has already cracked the bit. The red lines follow the scaling given by Equation~\eqref{poft}.

\begin{figure}[H]
\centering
\subfloat[]{
	\label{log_securecases}
	\includegraphics[width=3.15in]{CorrectguessvsBEP.pdf} } 
\subfloat[]{
	\label{log_crack}
	\includegraphics[width=3.2in]{CorrectguessvsBEPcomp.pdf} } 
\caption{Probabilities during the attack with single-bit resolution of Eve's measurements. (a) Probability that the exchange of the current key bit is still secure; (b) and probability that Eve has already cracked it. The histograms represent the simulation results, and the red lines represent the scaling given by Equation~\eqref{poft}.}
\end{figure}

\subsubsection{Attack Demonstration when Eve Knows Only One of the Sources}
\label{det_unidem}
At the unilateral parameter knowledge (see Section~\ref{unilateral}), Eve knows the root of Alice’s RNG, while the root of Bob’s RNG is unknown to her. Thus, we suppose she knows $U_\mathrm{A}(t)$ (like at the bilateral case), but not $U_\mathrm{B}(t)$. A realization of the wire voltage and current, $U_\mathrm{w}(t)$ and $I_\mathrm{w}(t)$, under the LH condition over 100 milliseconds, is displayed in Figure~\ref{Eve_wire_data}. Figure~\ref{Possible_voltagedrops} shows the hypothetical noise voltages generated by Eve's simulations across $R_\mathrm{L}$ and $R_\mathrm{H}$ via Ohm's Law.

\begin{figure}[H]
\centering
	\includegraphics[width=6in]{Eve_wire_data.pdf}
\caption{A realization of $U_\mathrm{w}(t)$ and $I_\mathrm{w}(t)$ (see Figure~\ref{figKLJN}) displayed over 100 milliseconds. Eve measures and records these data.\label{Eve_wire_data}}
\end{figure}

\begin{figure}[H]
\centering
	\includegraphics[width=6in]{Possible_voltagedrops.pdf}
\caption{Hypothetical noise voltage drops across $R_\mathrm{L}$ and $R_\mathrm{H}$ by Eve's current measurements and Ohm's law. These results are used in Equation~\eqref{UA} to calculate the hypothetical waveforms for $U_\mathrm{L,A}(t)$ and $U_\mathrm{H,A}(t)$.\label{Possible_voltagedrops}}
\end{figure}

Figure~\ref{Evecalc_vs_UA} shows Eve’s hypothetical waveforms for $U_\mathrm{L,A}(t)$ and $U_\mathrm{H,A}(t)$, which we denote as $U^\ast_\mathrm{R_L}(t)$ and $U^\ast_\mathrm{R_H}(t)$ (see Equation~\eqref{UA}), in comparison to her known $U_\mathrm{L,A}(t)$ and $U_\mathrm{H,A}(t)$. In this case, the waveform for $U^\ast_\mathrm{R_L}(t)$ is identical to that of $U_\mathrm{L,A}(t)$, thus Eve decides that Alice has chosen $R_\mathrm{L}$. A correlation plot is also shown in Figure~\ref{corr}, between (a) $U^\ast_\mathrm{R_L}(t)$ vs. $U_\mathrm{L,A}(t)$ and $U_\mathrm{H,A}(t)$, and (b) $U^\ast_\mathrm{R_H}(t)$ vs. $U_\mathrm{L,A}(t)$ and $U_\mathrm{H,A}(t)$. A one-to-one correlation between $U^\ast_\mathrm{R_L}(t)$ and $U_\mathrm{L,A}(t)$ indicates that Alice has chosen $R_\mathrm{L}$.

\begin{figure}[H]
\centering
	\includegraphics[width=6in]{Evecalc_vs_UA.pdf}
\caption{Eve’s hypothetical waveforms for $U_\mathrm{L,A}(t)$ and $U_\mathrm{H,A}(t)$, which we denote as $U^\ast_\mathrm{R_L}(t)$ and $U^\ast_\mathrm{R_H}(t)$ (see Equation~\eqref{UA}), in comparison to her known $U_\mathrm{L,A}(t)$ and $U_\mathrm{H,A}(t)$.\label{Evecalc_vs_UA}}
\end{figure}

\begin{figure}[H]
\centering
\subfloat[]{
	\label{corr_RL}
	\includegraphics[width=3.3in]{corr_RL.pdf} } 
\subfloat[]{
	\label{corr_RH}
	\includegraphics[width=3.3in]{corr_RH.pdf} } 
\caption{Correlation between (a) $U^\ast_\mathrm{R_L}(t)$ vs. $U_\mathrm{L,A}(t)$ and $U_\mathrm{H,A}(t)$, and (b) $U^\ast_\mathrm{R_H}(t)$ vs. $U_\mathrm{L,A}(t)$ and $U_\mathrm{H,A}(t)$. A one-to-one correlation between Eve's known $U_\mathrm{A}(t)$ and the hypothetical waveform for $U_\mathrm{L,A}(t)$ indicates that Alice has chosen $R_\mathrm{L}$.\label{corr}}
\end{figure}

Finally, Eve evaluates the measured mean-square voltage on the wire over the bit exchange period, shown in Figure~\ref{u2}. From that value, by using Equation~\eqref{meansquare}, she evaluates the parallel resultant $R_\mathrm{P}$ of the resistances of Alice and Bob. From $R_\mathrm{P}$ and $R_\mathrm{A}$, she can calculate $R_\mathrm{B}$. In this particular case, Bob has chosen $R_\mathrm{H}$, thus Eve has cracked the LH situation and the related secure bit value.

\begin{figure}[H]
\centering
	\includegraphics[width=4.5in]{u2.pdf}
\caption{The hypothetical and measured mean-square voltage generated by Eve. $U_\mathrm{HH,eff}^2$ is the hypothetical mean-square voltage in the HH case, $U_\mathrm{LL,eff}^2$ is the hypothetical mean-square voltage in the LL case, $U_\mathrm{HL,eff}^2$ is the hypothetical mean-square voltage in the HL case, and $U_\mathrm{LH,eff}^2$ is the hypothetical mean-square voltage in the LH case. $U_\mathrm{w,eff}^2$ is the measurement of the actual mean-square voltage.\label{u2}}
\end{figure}

\subsection{Transition}
\label{detRNGtransition}
This concludes the deterministic RNG attacks presented in this dissertation. Now, we move onto the statistical RNG attacks.

\section{Statistical RNG Attack against the KLJN Scheme}
\label{statRNGattack}

\subsection{Statistical Attack Protocol}
Two situations are introduced where Eve can use compromised RNGs to crack the KLJN scheme: one where Eve has partial knowledge of both Alice’s and Bob’s generators (bilateral knowledge), and another where Eve has partial knowledge of only Alice’s generator (unilateral knowledge).

\subsubsection{Bilateral Knowledge}
\label{statbilateral}
Eve has statistical knowledge of the amplitudes of the noise voltage generators $U_\mathrm{H,A}(t)$, $U_\mathrm{L,A}(t)$, $U_\mathrm{H,B}(t)$, and $U_\mathrm{L,B}(t)$ for each of Alice's and Bob's resistors, see Figure~\ref{figKLJN}. These noises are correlated with Alice's and Bob's corresponding noises. Eve then uses Equations~\eqref{Uw}, \eqref{Iw}, and \eqref{Pw} for the cross-correlation attacks shown below.

\paragraph{\it Cross-correlation attack utilizing Alice's/Bob's and Eve's channel voltages, currents and power}\mbox{}\\
\label{statCCCABW}
For the four possible resistor combinations, HL, LH, LL and HH, Eve sets up a simulator utilizing her noises (that are correlated with Alice's Bob's corresponding noises), and she records the resulting wire voltages $U_{\mathrm{HH}}(t)$, $U_{\mathrm{LL}}(t)$, $U_{\mathrm{HL}}(t)$, and $U_{\mathrm{LH}}(t)$. Then she evaluates the cross-correlation between the measured wire voltage $U_{\mathrm{w}}(t)$ of Alice and Bob, and the simulated ones. For example, in the HH simulated resistor situation, this is given by

\begin{equation}
CCC_{\mathrm{HH,U}}=\frac{\langle U_{\mathrm{w}}(t)U_{\mathrm{HH}}(t)\rangle}{U_{\mathrm{w}}U_{\mathrm{HH}}},\label{CCCHU}
\end{equation}

\noindent where $CCC_{\mathrm{HH,U}}$ is the cross-correlation coefficient between her simulated wire voltage $U_{\mathrm{HH}}(t)$ in the HH case and the \textit{measured} channel voltage $U_{\mathrm{w}}(t)$.

Finally, Eve guesses that the actual resistor situation is the one with the highest cross-correlation between the voltage on the wire and in Eve’s probing system.

Note, this protocol of cross-correlating the simulated and real wire data can also be repeated for the channel current $I_{\mathrm{w}}(t)$ and channel power $P_{\mathrm{w}}(t)$.

For the channel current protocol, she measures $I_{\mathrm{w}}(t)$ and evaluates the cross-correlation between the measured $I_{\mathrm{w}}(t)$ and her four simulated wire currents $I_{\mathrm{HH}}(t)$, $I_{\mathrm{LL}}(t)$, $I_{\mathrm{HL}}(t)$, and $I_{\mathrm{LH}}(t)$. In the HH example, this is given by

\begin{equation}
CCC_{\mathrm{HH,I}}=\frac{\langle I_{\mathrm{w}}(t)I_{\mathrm{HH}}(t) \rangle}{I_{\mathrm{w}}I_{\mathrm{HH}}},\label{CCCHI}
\end{equation}

\noindent where $CCC_{\mathrm{HH,I}}$ is the cross-correlation coefficient between her simulated wire voltage $I_{\mathrm{HH}}(t)$ in the HH case and the \textit{measured} channel current $I_{\mathrm{w}}(t)$.

Finally, similarly to the above voltage correlation attack, Eve guesses that the bit situation is the one with the highest cross-correlation between the current in the wire and in Eve's probing system.

For the channel power protocol, Eve has the measured $U_{\mathrm{w}}(t)$ and $I_{\mathrm{w}}(t)$ at her disposal. She uses her noises to simulate the four possible waveforms, $P_{\mathrm{HH}}(t)$, $P_{\mathrm{LL}}(t)$, $P_{\mathrm{HL}}(t)$, and $P_{\mathrm{LH}}(t)$, for the instantaneous power flow from Alice to Bob, and cross-correlates the with the actual measured $P_{\mathrm{w}}(t)$. In the HH example:

\begin{equation}
CCC_{\mathrm{HH,P}}=\frac{\langle P_{\mathrm{w}}(t)P_{\mathrm{HH}}(t)\rangle}{P_{\mathrm{w}}P_{\mathrm{HH}}},\label{CCCHP}
\end{equation}

\noindent where $P_{\mathrm{HH}}(t)$ is the simulated channel power in the HH case, and the measured power is given by Equation~\eqref{Pw}.

Finally, Eve guesses that the bit situation is the one with the highest cross-correlation between the power flows in the wire and in Eve's probing system.

\paragraph{\it Cross-correlation attack directly utilizing Alice's/Bob's and Eve's voltage sources}\mbox{}\\
\label{statCCCAB}
There is an alternative way for correlation attacks. Eve measures the wire voltage $U_{\mathrm{w}}(t)$ and wire current $I_{\mathrm{w}}(t)$ \cite{deterministicRNG,RNG}. Then, from $I_{\mathrm{w}}(t)$, she uses Ohm's law to calculate the hypothetical voltage drops on Alice’s/Bob’s possible choices of resistances $R_\mathrm{H}$ and $R_\mathrm{L}$. From that voltage drop, by using Kirchhoff's loop law, Eve calculates Alice's/Bob's hypothetical noise voltage amplitudes. With these data, she tests four hypotheses:

\noindent\begin{description}%[leftmargin=!,labelwidth=\widthof{The longest label}]
\item [Hypothesis (i):] Alice has chosen $R_{\textrm{L}}$
\item [Hypothesis (ii):] Alice has chosen $R_{\textrm{H}}$
\item [Hypothesis (iii):] Bob has chosen $R_{\textrm{L}}$
\item [Hypothesis (iv):] Bob has chosen $R_{\textrm{H}}$
\end{description}

With Hypothesis (i), to utilize Kirchhoff's loop law, using the same current direction (Alice $\rightarrow$ Bob) as with the power calculation in Equation~\eqref{Pw}, Eve takes the sum

\begin{equation}
U^\ast_{\mathrm{L,A}}(t)=U_{\mathrm{w}}(t)+I_{\mathrm{w}}(t)R_{\mathrm{L}}\label{EvesumAlice}
\end{equation}

\noindent to calculate the hypothetical value $U^\ast_{\mathrm{L,A}}(t)$ of Alice's noise $U_{\mathrm{L,A}}(t)$.

To test Hypothesis (i) she finds the cross-correlation between $U_{\mathrm{L,A}}(t)$ (see Figure~\ref{figKLJN}) and the $U^\ast_{\mathrm{L,A}}(t)$ determined by (Equation~\eqref{EvesumAlice}), given by

\begin{equation}
CCC_{\mathrm{LA}}=\frac{\langle U^\ast_{\mathrm{L,A}}(t)U_{\mathrm{L,A}}(t)\rangle}{U^\ast_{\mathrm{L,A}}U_{\mathrm{L,A}}}.\label{CCCLA}
\end{equation}

\noindent Then, with the same equation, she finds the cross-correlation coefficient between $U^\ast_{\mathrm{L,A}}(t)$ and $U_{\mathrm{H,A}}(t)$. If the former result yields the higher cross-correlation, then Eve has determined that Hypothesis (i) is correct; otherwise, Hypothesis (ii) is valid.

Similarly, at Bob's side, with Hypothesis (iii), Eve takes the difference

\begin{equation}
U^\ast_{\mathrm{L,B}}(t)=U_{\mathrm{w}}(t)-I_{\mathrm{w}}(t)R_{\mathrm{L}}\label{EvesumBob}
\end{equation}

\noindent to calculate the hypothetical value $U^\ast_{\mathrm{L,B}}(t)$ of Bob's noise $U_{\mathrm{L,B}}(t)$.

To test Hypothesis (iii) she finds the cross-correlation between $U_{\mathrm{L,B}}(t)$ (see Figure~\ref{figKLJN}) and the $U^\ast_{\mathrm{L,B}}(t)$ determined by Equation~\eqref{EvesumBob}, given by

\begin{equation}
CCC_{\mathrm{LB}}=\frac{\langle U^\ast_{\mathrm{L,B}}(t)U_{\mathrm{L,B}}(t)\rangle}{U^\ast_{\mathrm{L,B}}U_{\mathrm{L,B}}}.\label{CCCLB}
\end{equation}

\noindent Then, with the same equation, she finds the cross-correlation coefficient between $U^\ast_{\mathrm{L,B}}(t)$ and $U_{\mathrm{H,B}}(t)$. If the former result yields the higher cross-correlation, then Eve has determined that Hypothesis (iii) is correct; otherwise, Hypothesis (iv) is valid.

\subsubsection{Unilateral Knowledge}
Eve has partial knowledge of only Alice’s noises, that is, the noise generator outputs of Alice’s resistors, $U_{\mathrm{L,A}}(t)$ and $U_{\mathrm{H,A}}(t)$. Bob’s generator voltages are completely unknown to her. The attack methods described in Section~\ref{statbilateral} work even here with a minor modification as described below.

\paragraph{\it Cross-correlations between Alice's/Bob's and Eve's channel voltages, currents and power}\mbox{}\\
Eve generates two independent "dummy" thermal noises to substitute for Bob's unknown noise voltages $U_{\mathrm{H,B}}(t)$ and $U_{\mathrm{L,B}}(t)$. Then, she uses the same protocol as the bilateral case (see Section~\ref{statbilateral}): she measures $U_{\mathrm{w}}(t)$ and $I_{\mathrm{w}}(t)$, determines $P_{\mathrm{w}}(t)$ from Equation~\eqref{Pw}, and uses Equations~\eqref{CCCHU}-\eqref{CCCHP} to find the cross-correlation between her four simulated $U_{\mathrm{w}}(t)$, $I_{\mathrm{w}}(t)$, and $P_{\mathrm{w}}(t)$, and the measured $U_{\mathrm{w}}(t)$, $I_{\mathrm{w}}(t)$, and $P_{\mathrm{w}}(t)$.

\paragraph{\it Cross-correlations between Alice's and Eve's voltage sources}\mbox{}\\
\label{statCCCAB_uni}
With $U_{\mathrm{L,A}}(t)$ and $U_{\mathrm{H,A}}(t)$ partially known, Eve uses a protocol corresponding to the bilateral case (see Section~\ref{statbilateral}): she measures $U_{\mathrm{w}}(t)$ and $I_{\mathrm{w}}(t)$ \cite{deterministicRNG,RNG}. Then, from $I_{\mathrm{w}}(t)$, she calculates the hypothetical voltage drops on Alice’s possible choice of resistances $R_{\mathrm{H}}$ and $R_{\mathrm{L}}$. With these data, she tests two hypotheses:

\noindent\begin{description}%[leftmargin=!,labelwidth=\widthof{The longest label}]
\item [Hypothesis (i):] Alice has chosen $R_{\textrm{L}}$
\item [Hypothesis (ii):] Alice has chosen $R_{\textrm{H}}$.
\end{description}

Note that, in the bilateral case, she had knowledge of Bob’s noises, thus she could form four hypotheses. In the unilateral case, she has knowledge of only Alice’s generator voltages, therefore she can form only two hypotheses.

With Hypothesis (i), Eve uses Equation~\eqref{EvesumAlice} to find $U^\ast_{\mathrm{L,A}}(t)$. Then, she uses Equation~\eqref{CCCLA} to find the cross-correlation between $U_{\mathrm{L,A}}(t)$ and $U^\ast_{\mathrm{L,A}}(t)$, and then the cross-correlation between $U^\ast_{\mathrm{L,A}}(t)$ and $U_{\mathrm{H,A}}(t)$. If the former result yields the higher cross-correlation, then Eve has determined that Hypothesis (i) is correct; otherwise, Hypothesis (ii) is valid.

The extra step that is needed to add to the protocol described in Section~\ref{statCCCAB} is as follows: with Alice's chosen resistance known, Eve does the same exact KLJN protocol as Alice {see Section~\ref{KLJN}): she evaluates the measured mean-square voltage on the wire over the whole bit exchange period. From that value, by using Equation~\eqref{meansquare}, she evaluates the bit situation (see Figure~\ref{threelevels}). Thus she has cracked the KLJN scheme \cite{RNG}.

\subsection{Demonstration}
\label{statRNGresults}

The noise generation is the same as in Sections~\ref{OGnoisegen} and \ref{EvenoisegenM}.


\subsubsection{Attack demonstration when Eve knows both noises (bilateral attacks)}

\paragraph{\it Bilateral attack demonstration utilizing cross-correlations between Alice's/Bob's and Eve's wire voltages, currents and powers}\mbox{}\\
\label{bilatchannel}

Computer simulations were executed with MATLAB, and each simulation was averaged over 1000 runs, see Tables~\ref{bilat_channel_table}-\ref{unilat_sources_table}. During the attacks, the sample size (number of time steps) is 1000, and the KLJN system is kept in the LH state. A realization of the wire voltage, current, and power, $U_\mathrm{w}(t)$, $I_\mathrm{w}(t)$, and $P_\mathrm{w}(t)$, under the LH condition over 100 milliseconds is displayed in Figure~\ref{Eve_wire_data_power}.

\begin{figure}[H]
\centering
	\includegraphics[width=6in]{Eve_wire_data_power.pdf}
\caption{A realization of $U_\mathrm{w}(t)$, $I_\mathrm{w}(t)$, (see Figure~\ref{figKLJN}) and $P_\mathrm{w}(t)$ (see Equation~\eqref{Pw}) for the LH situation displayed over 100 milliseconds \cite{RNG}. Eve measures and records these data.\label{Eve_wire_data_power}}
\end{figure}

A visual example of the correlations between Eve's \textit{measured} channel voltage, $U_\mathrm{w}(t)$, and her four \textit{simulated} channel voltages, $U_\mathrm{HH}(t)$, $U_\mathrm{LL}(t)$, $U_\mathrm{HL}(t)$, and $U_\mathrm{LH}(t)$, at $M=1$ (see Section~\ref{EvenoisegenM}), is shown in Figure~\ref{bilateral_channel_corr}. The highest correlation is the LH case, thus Eve guesses that the secure resistance situation is LH.

\begin{figure}[H]
\centering
	\includegraphics[width=6in]{bilateral_channel_corr.pdf}
\caption{Correlation between Eve's \textit{measured} channel voltage, $U_\mathrm{w}(t)$, and her four \textit{simulated} channel voltages, $U_\mathrm{HH}(t)$, $U_\mathrm{LL}(t)$, $U_\mathrm{HL}(t)$, and $U_\mathrm{LH}(t)$ at $M=1$.\label{bilateral_channel_corr}}
\end{figure}

The results of the attack are shown in Table~\ref{bilat_channel_table}. The HL situation of Eve has zero cross-correlation with Eve's probe signals because, in this case, Alice/Bob and Eve do not have a common noise. In all the other cases, they have at least one mutual noise. In the LH attack situation, both noises are common, thus they yield the highest cross-correlation with Eve's LH probe, therefore Eve guesses that the secure resistance situation is LH.

Using the correlations between the voltages for the attack yielded the highest probability $p$ of successful guessing, and the correlations between the powers yielded the lowest one. This is because power is the product of voltage and current (see Equation~\eqref{Pw}), and the inaccuracies in both the voltage and current correlations affect the power correlations.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[htbp!]
\centering
\caption{Simulation of the average cross-correlation coefficient, $CCC$ (see Equations~\eqref{CCCHU}-\eqref{CCCHP}), Eve’s average $p$ of correctly guessing the LH bit situations, and standard deviation $\sigma$ at varying multipliers $M$ (see Section~\ref{EvenoisegenM}). As $M$ increases, which implies increasing differences between the noises of Alice/Bob and Eve’s probing noises, the cross-correlation decreases. Yet, in each case of the present situation, the LH case yields the highest correlation. Thus, Eve guesses that LH is the secure bit situation. The correlations $CCC_\mathrm{u}$ between the voltages yielded $p_\mathrm{u}$, which had the highest probability $p$ of successful guessing, and the correlations $CCC_\mathrm{p}$ between the powers yielded the lowest $p$. This is because power is the product of voltage and current (see Equation~\eqref{Pw}), and the inaccuracies in both the voltage and current correlations affect the power correlations.}
\label{bilat_channel_table}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c}
\cline{1-11}

\begin{tabular}[c]{@{}c@{}}Eve's \\ probing \\ bit\end{tabular} & $M$                    & $CCC_\mathrm{u}$     & $p_\mathrm{u}$               & $\sigma_\mathrm{u}$           & $CCC_\mathrm{i}$     & $p_\mathrm{i}$               & $\sigma_\mathrm{i}$           & $CCC_\mathrm{p}$     & $p_\mathrm{p}$               & $\sigma_\mathrm{p}$           &  \\ \cline{1-11}
HH                & \multirow{4}{*}{0}   & 0.21314  & \multirow{3}{*}{} & \multirow{3}{*}{} & 0.67455  & \multirow{3}{*}{} & \multirow{3}{*}{} & 0.28482  & \multirow{3}{*}{} & \multirow{3}{*}{} &  \\ \cline{1-1} \cline{3-3} \cline{6-6} \cline{9-9}
LL                &                      & 0.67377  &                   &                   & 0.21317  &                   &                   & 0.28502  &                   &                   &  \\ \cline{1-1} \cline{3-3} \cline{6-6} \cline{9-9}
HL                &                      & -0.00118 &                   &                   & 0.00128  &                   &                   & -0.00126 &                   &                   &  \\ \cline{1-1} \cline{3-11}
LH                &                      & 1        & 1                 & 0                 & 1        & 1                 & 0                 & 1        & 1                 & 0                 &  \\ \cline{1-11}
HH                & \multirow{4}{*}{0.1} & 0.21087  & \multirow{3}{*}{} & \multirow{3}{*}{} & 0.67048  & \multirow{3}{*}{} & \multirow{3}{*}{} & 0.28198  & \multirow{3}{*}{} & \multirow{3}{*}{} &  \\ \cline{1-1} \cline{3-3} \cline{6-6} \cline{9-9}
LL                &                      & 0.67090  &                   &                   & 0.21326  &                   &                   & 0.28573  &                   &                   &  \\ \cline{1-1} \cline{3-3} \cline{6-6} \cline{9-9}
HL                &                      & -0.00030 &                   &                   & -0.00007 &                   &                   & 0.00095  &                   &                   &  \\ \cline{1-1} \cline{3-11}
LH                &                      & 0.99504  & 1                 & 0                 & 0.99505  & 1                 & 0                 & 0.99005  & 1                 & 0                 &  \\ \cline{1-11}
HH                & \multirow{4}{*}{0.5} & 0.18975  & \multirow{3}{*}{} & \multirow{3}{*}{} & 0.60201  & \multirow{3}{*}{} & \multirow{3}{*}{} & 0.23101  & \multirow{3}{*}{} & \multirow{3}{*}{} &  \\ \cline{1-1} \cline{3-3} \cline{6-6} \cline{9-9}
LL                &                      & 0.60349  &                   &                   & 0.19047  &                   &                   & 0.23089  &                   &                   &  \\ \cline{1-1} \cline{3-3} \cline{6-6} \cline{9-9}
HL                &                      & -0.00023 &                   &                   & -0.00090 &                   &                   & -0.00114 &                   &                   &  \\ \cline{1-1} \cline{3-11}
LH                &                      & 0.89457  & 1                 & 0                 & 0.89441  & 1                 & 0                 & 0.79926  & 1                 & 0                 &  \\ \cline{1-11}
HH                & \multirow{4}{*}{1}   & 0.15004  & \multirow{3}{*}{} & \multirow{3}{*}{} & 0.47631  & \multirow{3}{*}{} & \multirow{3}{*}{} & 0.14297  & \multirow{3}{*}{} & \multirow{3}{*}{} &  \\ \cline{1-1} \cline{3-3} \cline{6-6} \cline{9-9}
LL                &                      & 0.47705  &                   &                   & 0.15241  &                   &                   & 0.14315  &                   &                   &  \\ \cline{1-1} \cline{3-3} \cline{6-6} \cline{9-9}
HL                &                      & 0.00082  &                   &                   & 0.00074  &                   &                   & 0.00061  &                   &                   &  \\ \cline{1-1} \cline{3-11}
LH                &                      & 0.70664  & 1                 & 0                 & 0.70667  & 1                 & 0                 & 0.49926  & 1                 & 0                 &  \\ \cline{1-11}
HH                & \multirow{4}{*}{1.5} & 0.11814  & \multirow{3}{*}{} & \multirow{3}{*}{} & 0.37380  & \multirow{3}{*}{} & \multirow{3}{*}{} & 0.08931  & \multirow{3}{*}{} & \multirow{3}{*}{} &  \\ \cline{1-1} \cline{3-3} \cline{6-6} \cline{9-9}
LL                &                      & 0.37390  &                   &                   & 0.11798  &                   &                   & 0.08669  &                   &                   &  \\ \cline{1-1} \cline{3-3} \cline{6-6} \cline{9-9}
HL                &                      & 0.00022  &                   &                   & -0.00024 &                   &                   & -0.00141 &                   &                   &  \\ \cline{1-1} \cline{3-11}
LH                &                      & 0.55434  & 1                 & 0                 & 0.55473  & 1                 & 0                 & 0.30762  & 1                 & 0                 &  \\ \cline{1-11}
HH                & \multirow{4}{*}{5}   & 0.04021  & \multirow{3}{*}{} & \multirow{3}{*}{} & 0.13280  & \multirow{3}{*}{} & \multirow{3}{*}{} & 0.01158  & \multirow{3}{*}{} & \multirow{3}{*}{} &  \\ \cline{1-1} \cline{3-3} \cline{6-6} \cline{9-9}
LL                &                      & 0.13142  &                   &                   & 0.03961  &                   &                   & 0.01000  &                   &                   &  \\ \cline{1-1} \cline{3-3} \cline{6-6} \cline{9-9}
HL                &                      & -0.00069 &                   &                   & 0.00087  &                   &                   & -0.00052 &                   &                   &  \\ \cline{1-1} \cline{3-11}
LH                &                      & 0.19490  & 1                 & 0                 & 0.19525  & 0.996             & 0.0144            & 0.03830  & 0.756             & 0.0144            &  \\ \cline{1-11}
HH                & \multirow{4}{*}{10}  & 0.02200  & \multirow{3}{*}{} & \multirow{3}{*}{} & 0.06581  & \multirow{3}{*}{} & \multirow{3}{*}{} & 0.00266  & \multirow{3}{*}{} & \multirow{3}{*}{} &  \\ \cline{1-1} \cline{3-3} \cline{6-6} \cline{9-9}
LL                &                      & 0.06692  &                   &                   & 0.02130  &                   &                   & 0.00525  &                   &                   &  \\ \cline{1-1} \cline{3-3} \cline{6-6} \cline{9-9}
HL                &                      & 0.00064  &                   &                   & -0.00102 &                   &                   & 0.00090  &                   &                   &  \\ \cline{1-1} \cline{3-11}
LH                &                      & 0.09905  & 0.977             & 0.0034            & 0.09878  & 0.907             & 0.0111            & 0.01244  & 0.613             & 0.0209            &  \\ \cline{1-11}
\end{tabular}
\end{table}

\paragraph{\it Bilateral attack demonstration utilizing cross-correlations among the voltage sources}\mbox{}\\
\label{bilatsources_demo}

Eve uses Equation~\eqref{EvesumAlice} to find $U^\ast_{\mathrm{L,A}}(t)$, Equation~\eqref{CCCLA} to find the cross-correlation between $U^\ast_{\mathrm{L,A}}(t)$ and $U_{\mathrm{L,A}}(t)$, Equation~\eqref{EvesumBob} to find $U^\ast_{\mathrm{L,B}}(t)$, and Equation~\eqref{CCCLB} to find the cross-correlation between $U^\ast_{\mathrm{L,B}}(t)$ and $U_{\mathrm{L,B}}(t)$. 

A visual example of the correlations between (a) $U^\ast_\mathrm{L,A}(t)$ and $U_\mathrm{L,A}(t)$, $U^\ast_\mathrm{L,A}(t)$ and $U_\mathrm{H,A}(t)$, and (b) $U^\ast_\mathrm{L,B}(t)$ and $U_\mathrm{L,B}(t)$, $U^\ast_\mathrm{L,B}(t)$ and $U_\mathrm{H,B}(t)$, is shown in Figure~\ref{bilateral_AB_corr}. The highest correlation on Alice's side is with $U^\ast_\mathrm{L,A}(t)$, and the highest correlation on Bob's side is with $U_\mathrm{H,B}(t)$, thus Eve guesses that Alice has $R_\mathrm{L}$ and Bob has $R_\mathrm{H}$.

\begin{figure}[H]
\centering
\subfloat[]{
	\label{corr_UA}
	\includegraphics[width=3in]{bilateral_UA_corr.pdf} } 
\subfloat[]{
	\label{corr_UB}
	\includegraphics[width=3in]{bilateral_UB_corr.pdf} } 
\caption{Correlation between (a) $U^\ast_{\mathrm{L,A}}(t)$ vs. $U_\mathrm{L,A}(t)$ and $U_\mathrm{H,A}(t)$, and (b) $U^\ast_{\mathrm{L,B}}(t)$ vs. $U_\mathrm{L,B}(t)$ and $U_\mathrm{H,B}(t)$. The highest correlation on Alice's side is with $U^\ast_\mathrm{L,A}(t)$, and the highest correlation on Bob's side is with $U_\mathrm{H,B}(t)$, thus Eve guesses that Alice has $R_\mathrm{L}$ and Bob has $R_\mathrm{H}$.\label{bilateral_AB_corr}}
\end{figure}

A simulation results of the cross correlation for each bit case is displayed in Table~\ref{bilat_sources_table}. As the multiplier $M$ in the superposition increases (see Section~\ref{EvenoisegenM}), the correlations decrease. Yet, in each case at the present (LH) situation, the highest correlation ended up being the LH case, thus Eve has decided that LH is the secure resistance situation.

\begin{table}[htbp!]
\centering
\caption{Simulation of the cross-correlation coefficients $CCC$ at the attack described in Section~\ref{statCCCAB} (see Equations~\eqref{CCCLA} and \eqref{CCCLB}), Eve’s average correct-guessing probability $p$, and standard deviation $\sigma$ at varying multipliers $M$ (see Section~\ref{EvenoisegenM}). As $M$ increases, which implies increasing differences between the noises of Alice/Bob and Eve’s probing noises, the cross-correlation decreases. Yet, in each case of the present situation, the $R_\mathrm{L}$ hypothesis yields the highest cross-correlation with Alice's noise. Thus, Eve guesses that Alice has $R_\mathrm{L}$. The same procedure done for Bob's noise results in the highest cross-correlation for the $R_\mathrm{H}$ hypothesis at Bob's side.}
\label{bilat_sources_table}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
$M$   & $CCC_\mathrm{LA} (R_\mathrm{L})$ & $CCC_\mathrm{LA} (R_\mathrm{H})$ & $CCC_\mathrm{LB} (R_\mathrm{L})$   & $CCC_\mathrm{LB} (R_\mathrm{H})$ & $p$     & $\sigma$  \\ \hline
0   & 1         & -0.03331  & -0.00092  & 0.57727    & 1     & 0      \\ \hline
0.1 & 0.99504   & 0.00948   & 0.00031   & 0.55856    & 1     & 0      \\ \hline
0.5 & 0.89451   & 0.01440   & 0.00063   & 0.51939    & 1     & 0      \\ \hline
1   & 0.70682   & -0.05075  & 0.00140   & 0.40084    & 1     & 0      \\ \hline
1.5 & 0.55430   & -0.02511  & 0.00004   & 0.31684    & 1     & 0      \\ \hline
5   & 0.19496   & -0.03176  & -0.00088  & 0.14445    & 0.995 & 0.0022 \\ \hline
10  & 0.09949   & -0.02127  & -0.00009  & 0.01611    & 0.894 & 0.0095 \\ \hline
\end{tabular}
\end{table}

\subsubsection{Attack demonstration when Eve knows only one of the sources (unilateral attacks)}

\paragraph{\it Unilateral attack demonstration utilizing cross-correlations between Alice's/Bob's and Eve's wire voltages, currents and powers}\mbox{}\\

Like the bilateral results (see Section~\ref{bilatchannel}), the HL situation of Eve has zero cross-correlation with Eve's probe signals because, in this case, Alice/Bob, and Eve do not have a common noise. In all the other cases, they have at least one mutual noise. In the LH probe attack, both noises are common, thus they yield the highest cross-correlation with Eve's LH probe, therefore Eve guesses that the secure resistance situation is LH, see Table~\ref{bilat_sources_table}.

Using the correlations between the voltages for the attack yielded the highest probability $p$ of successful guessing, and the correlations between the powers yielded the lowest one. This is because power is the product of voltage and current (see Equation~\eqref{Pw}), and the inaccuracies in both the voltage and current correlations affect the power correlations.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[htbp!]
\centering
\caption{Simulation of the cross-correlation coefficient, $CCC$ (see Equations~\eqref{CCCHU}-\eqref{CCCHP}), Eve’s average $p$ of correctly guessing the LH bit situations, and standard deviation $\sigma$ at varying multipliers $M$ (see Section~\ref{EvenoisegenM}). As $M$ increases, which implies increasing differences between the noises of Alice/Bob and Eve’s probing noises, the cross-correlation decreases. Yet, in each case of the present situation, the LH case yields the highest correlation. Thus, Eve guesses that LH is the secure bit situation. The correlations $CCC_\mathrm{u}$ between the voltages yielded $p_\mathrm{u}$, which had the highest probability $p$ of successful guessing, and the correlations $CCC_\mathrm{p}$ between the powers yielded the lowest $p$. This is because power is the product of voltage and current (see Equation~\eqref{Pw}), and the inaccuracies in both the voltage and current correlations affect the power correlations.}
\label{unilat_channel_table}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c}
\cline{1-11}
\begin{tabular}[c]{@{}c@{}}Eve's \\ probing \\ bit\end{tabular} & $M$                    & $CCC_\mathrm{u}$     & $p_\mathrm{u}$               & $\sigma_\mathrm{u}$           & $CCC_\mathrm{i}$     & $p_\mathrm{i}$               & $\sigma_\mathrm{i}$           & $CCC_\mathrm{p}$     & $p_\mathrm{p}$               & $\sigma_\mathrm{p}$           &  \\ \cline{1-11}
HH                & \multirow{4}{*}{0}   & -0.00166                   & \multirow{3}{*}{}        & \multirow{3}{*}{}            & 0.00018                    & \multirow{3}{*}{}        & \multirow{3}{*}{}            & -0.00055                   & \multirow{3}{*}{}        & \multirow{3}{*}{}            &                      \\ \cline{1-1} \cline{3-3} \cline{6-6} \cline{9-9}
LL                &                      & 0.67432                    &                          &                              & 0.08975                    &                          &                              & 0.16311                    &                          &                              &                      \\ \cline{1-1} \cline{3-3} \cline{6-6} \cline{9-9}
HL                &                      & 0.00055                    &                          &                              & 0.00084                    &                          &                              & -0.00193                   &                          &                              &                      \\ \cline{1-1} \cline{3-11}
LH                &                      & 0.90898                    & 1                        & 0                            & 0.21237                    & 0.995                    & 0.0016                       & 0.28506                    & 0.982                    & 0.0042                       &                      \\ \cline{1-11}
HH                & \multirow{4}{*}{0.1} & -0.00027                   & \multirow{3}{*}{}        & \multirow{3}{*}{}            & -0.00048                   & \multirow{3}{*}{}        & \multirow{3}{*}{}            & 0.00198                    & \multirow{3}{*}{}        & \multirow{3}{*}{}            &                      \\ \cline{1-1} \cline{3-3} \cline{6-6} \cline{9-9}
LL                &                      & 0.67119                    &                          &                              & 0.09030                    &                          &                              & 0.16500                    &                          &                              &                      \\ \cline{1-1} \cline{3-3} \cline{6-6} \cline{9-9}
HL                &                      & 0.00051                    &                          &                              & -0.00006                   &                          &                              & 0.00048                    &                          &                              &                      \\ \cline{1-1} \cline{3-11}
LH                &                      & 0.90462                    & 1                        & 0                            & 0.21337                    & 0.995                    & 0.0026                       & 0.28580                    & 0.980                    & 0.0044                       &                      \\ \cline{1-11}
HH                & \multirow{4}{*}{0.5} & 0.00022                    & \multirow{3}{*}{}        & \multirow{3}{*}{}            & 0.00049                    & \multirow{3}{*}{}        & \multirow{3}{*}{}            & 0.00224                    & \multirow{3}{*}{}        & \multirow{3}{*}{}            &                      \\ \cline{1-1} \cline{3-3} \cline{6-6} \cline{9-9}
LL                &                      & 0.60249                    &                          &                              & 0.08149                    &                          &                              & 0.13370                    &                          &                              &                      \\ \cline{1-1} \cline{3-3} \cline{6-6} \cline{9-9}
HL                &                      & -0.00168                   &                          &                              & -0.00165                   &                          &                              & 0.00062                    &                          &                              &                      \\ \cline{1-1} \cline{3-11}
LH                &                      & 0.81357                    & 1                        & 0                            & 0.18865                    & 0.983                    & 0.0034                       & 0.23146                    & 0.962                    & 0.0049                       &                      \\ \cline{1-11}
HH                & \multirow{4}{*}{1}   & -0.00081                   & \multirow{3}{*}{}        & \multirow{3}{*}{}            & 0.00079                    & \multirow{3}{*}{}        & \multirow{3}{*}{}            & -0.0000                    & \multirow{3}{*}{}        & \multirow{3}{*}{}            &                      \\ \cline{1-1} \cline{3-3} \cline{6-6} \cline{9-9}
LL                &                      & 0.47610                    &                          &                              & 0.06526                    &                          &                              & 0.08290                    &                          &                              &                      \\ \cline{1-1} \cline{3-3} \cline{6-6} \cline{9-9}
HL                &                      & -0.00029                   &                          &                              & 0.00009                    &                          &                              & 0.00092                    &                          &                              &                      \\ \cline{1-1} \cline{3-11}
LH                &                      & 0.64237                    & 1                        & 0                            & 0.15093                    & 0.929                    & 0.0132                       & 0.14373                    & 0.926                    & 0.0062                       &                      \\ \cline{1-11}
HH                & \multirow{4}{*}{1.5} & -0.00046                   & \multirow{3}{*}{}        & \multirow{3}{*}{}            & -0.00097                   & \multirow{3}{*}{}        & \multirow{3}{*}{}            & 0.00001                    & \multirow{3}{*}{}        & \multirow{3}{*}{}            &                      \\ \cline{1-1} \cline{3-3} \cline{6-6} \cline{9-9}
LL                &                      & 0.37480                    &                          &                              & 0.04921                    &                          &                              & 0.04924                    &                          &                              &                      \\ \cline{1-1} \cline{3-3} \cline{6-6} \cline{9-9}
HL                &                      & 0.00159                    &                          &                              & 0.00003                    &                          &                              & -0.00016                   &                          &                              &                      \\ \cline{1-1} \cline{3-11}
LH                &                      & 0.50383                    & 1                        & 0                            & 0.11863                    & 0.859                    & 0.0133                       & 0.08675                    & 0.827                    & 0.0116                       &                      \\ \cline{1-11}
HH                & \multirow{4}{*}{5}   & -0.00018                   & \multirow{3}{*}{}        & \multirow{3}{*}{}            & 0.00094                    & \multirow{3}{*}{}        & \multirow{3}{*}{}            & 0.00088                    & \multirow{3}{*}{}        & \multirow{3}{*}{}            &                      \\ \cline{1-1} \cline{3-3} \cline{6-6} \cline{9-9}
LL                &                      & 0.13188                    &                          &                              & 0.01730                    &                          &                              & 0.00728                    &                          &                              &                      \\ \cline{1-1} \cline{3-3} \cline{6-6} \cline{9-9}
HL                &                      & 0.00010                    &                          &                              & 0.00168                    &                          &                              & -0.00036                   &                          &                              &                      \\ \cline{1-1} \cline{3-11}
LH                &                      & 0.17768                    & 1                        & 0                            & 0.04152                    & 0.637                    & 0.0157                       & 0.01052                    & 0.561                    & 0.0143                       &                      \\ \cline{1-11}
HH                & \multirow{4}{*}{10}  & 0.00058                    & \multirow{3}{*}{}        & \multirow{3}{*}{}            & -0.00017                   & \multirow{3}{*}{}        & \multirow{3}{*}{}            & -0.00088                   & \multirow{3}{*}{}        & \multirow{3}{*}{}            &                      \\ \cline{1-1} \cline{3-3} \cline{6-6} \cline{9-9}
LL                &                      & 0.06566                    &                          &                              & 0.00989                    &                          &                              & 0.00180                    &                          &                              &                      \\ \cline{1-1} \cline{3-3} \cline{6-6} \cline{9-9}
HL                &                      & -0.00108                   &                          &                              & 0.00121                    &                          &                              & -0.00096                   &                          &                              &                      \\ \cline{1-1} \cline{3-11}
LH                &                      & 0.08992                    & 0.978                    & 0.0055                       & 0.02084                    & 0.604                    & 0.0134                       & 0.00307                    & 0.523                    & 0.0170                       &                      \\ \cline{1-11}
\end{tabular}
\end{table}

Finally, Eve evaluates the measured mean-square voltage on the wire over the bit exchange period. From that value, by using Equation~\eqref{meansquare}, she evaluates the parallel resultant $R_\mathrm{P}$ of the resistances of Alice and Bob. From $R_\mathrm{P}$ and $R_\mathrm{A}$, she can calculate $R_\mathrm{B}$. In this particular case, from the mean-square voltage Eve will learn that the actual situation is LH thus Bob has chosen $R_\mathrm{H}$ because Alice has $R_\mathrm{L}$ \cite{RNG}.

Alternatively, since she knows Alice's resistance, she can use the mean-square voltage to determine the secure bit situation and thus crack the KLJN scheme.

\paragraph{\it Unilateral attack demonstration utilizing cross-correlations among the voltage sources}\mbox{}\\
\label{unilatsources_demo}

Eve uses (Equation~\eqref{EvesumAlice}) to find $U^\ast_\mathrm{L,A}(t)$ and (Equation~\eqref{CCCLA}) to find the cross-correlation between $U^\ast_\mathrm{L,A}(t)$ and $U_\mathrm{L,A}(t)$. A simulation results of the cross correlation for each bit case is displayed in Table~\ref{unilat_sources_table}. As the multiplier $M$ increases (see Section~\ref{EvenoisegenM}), the correlation decreases, yet the highest correlation always ended up being the LH case, thus Eve has decided that LH is the secure resistance situation.

\begin{table}[htbp!]
\centering
\caption{A realization of the cross-correlation coefficient, $CCC$ (see Equation~\eqref{CCCLA}), Eve’s average correct-guessing probability $p$, and standard deviation $\sigma$ at varying multipliers $M$ (see Section~\ref{EvenoisegenM}). As $M$ increases, which implies increasing differences between the noises of Alice/Bob and Eve’s probing noises, the cross-correlation decreases. Yet, the $R_\mathrm{L}$ case yields the highest correlation. Thus, Eve guesses that Alice has $R_\mathrm{L}$.}
\label{unilat_sources_table}
\begin{tabular}{|c|c|c|c|c|}
\hline
$M$   & $CCC_\mathrm{LA} (R_\mathrm{L})$ & $CCC_\mathrm{LA} (R_\mathrm{H})$ & $p$     & $\sigma$  \\ \hline
0   & 1         & -0.03331 & 1     & 0      \\ \hline
0.1 & 0.99504   & 0.00948   & 1     & 0      \\ \hline
0.5 & 0.89451   & 0.01440   & 1     & 0      \\ \hline
1   & 0.70682   & -0.05075  & 1     & 0      \\ \hline
1.5 & 0.55430   & -0.02511  & 1     & 0      \\ \hline
5   & 0.19496   & -0.03176  & 1     & 0      \\ \hline
10  & 0.09949   & -0.02127  & 0.989 & 0.0022 \\ \hline
\end{tabular}
\end{table}

Finally, Eve evaluates the measured mean-square voltage on the wire over the bit exchange period. From that value, by using Equation~\eqref{meansquare}, she evaluates the parallel resultant $R_\mathrm{P}$ of the resistances of Alice and Bob. From $R_\mathrm{P}$ and $R_\mathrm{A}$, she can calculate $R_\mathrm{B}$. In this particular case, from the mean-square voltage, Eve will learn that the actual situation is LH, thus Bob has chosen $R_\mathrm{H}$ because Alice has $R_\mathrm{L}$ \cite{RNG}.

\subsection{Transition}
\label{statRNGtransition}
This concludes the RNG attacks presented in this dissertation. As a take-home message, the security of the KLJN scheme requires the RNG outputs to appear truly random for Eve. Now, we move onto the zero-crossing attack.


==> data/abstract_fallback.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Fall 2016.  
%
%
%  Author: Sean Zachary Roberson
%  Version 3.17.09
%  Last Updated: 9/21/2017
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                           ABSTRACT 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\chapter*{ABSTRACT}
\addcontentsline{toc}{chapter}{ABSTRACT} % Needs to be set to part, so the TOC doesnt add 'CHAPTER ' prefix in the TOC.

\pagestyle{plain} % No headers, just page numbers
\pagenumbering{roman} % Roman numerals
\setcounter{page}{2}

\indent This is the first numbered page, lower case Roman numberal (ii). Page numbers are outside the prescribed margins, at the bottom of the page and centered; everything else is inside the margins.No bold on this page (Exception: heading ABSTRACT is bold if major headings are bold. \emph{This \LaTeX ~ template applies to this exception}).

Text begins two double spaces below the major heading. Recommended length of text is no more than 350 words. Vertical spacing is double spaced or space-and-a-half. (\emph{This \LaTeX ~ template applies double space for this ABSTRACT.}) The same margin settings and text alignment are followed else where in this thesis. There should be no numbered references or formal citations in ABSTRACT.

The content of this ABSTRACT provides a complete, succinct snapshot of the research, addressing the purpose, methods, results, and conclusions of the research. As a result, it should stand alone without any formal citations or references to chapters/sections of the work. To accomodate with a variety of online database, images or complex equations should also be avoided.

The next pages are Dedication, Acknowledgments, Contributors and Funding Sources, and Nomenclature. Of these, Contributors and Funding Sources is required. The rest are optional.





A secure key distribution (exchange) scheme is unconditionally secure if it is unbreakable against arbitrary technological improvements of computing power and/or any development of new algorithms. Software based secure key exchange algorithms utilize mathematical schemes that are crackable but they are time consuming to crack by known algorithms and currently available computing power thus they are neither unconditionally secure nor future proof. Neither are unconditionally secure the recent "Post-Quantum" algorithmic schemes where the name implies that the mathematically hard problems utilized by these solutions cannot be cracked by known quantum computing algorithms yet they maybe crackable by other computational schemes (such as Noise-based Logic) or yet-to-be found classical or quantum algorithms.

There are only two families of experimentally realized and tested unconditionally secure key distribution technologies: Quantum Key Distribution (QKD), the base of quantum cryptography, which
utilizes quantum physical photonic features; and the Kirchhoff-Law-Johnson-Noise (KLJN) system that is based on classical statistical physics (fluctuation-dissipation theorem). Both the QKD and KLJN schemes count also as "Post-Quantum" hardware solutions, because they are resilient against any (past and future) computing schemes including quantum computers, but only the KLJN scheme can be integrated on chips with currently available technology to offer unconditional security of communication within computers and instruments.

Very recently, National Security Agency (NSA) has made a public statement: "NSA does not recommend the usage of quantum key distribution and quantum cryptography for securing the transmission of data in National Security Systems (NSS)...". While we have reservations about this NSA statement, it inherently brings KLJN up for further considerations.

The first focus topic of this thesis is the vulnerability of the Kirchhoff-Law-Johnson-Noise (KLJN) secure key exchanger to compromised random number generator(s) even if these random numbers are used solely to generate the noises emulating the Johnson noise of Alice's and Bob's resistors.

The first RNG attacks shown are deterministic in the sense that Eve's knowledge of Alice's and/or Bob's random numbers is basically deterministic. Moreover, no statistical evaluation is needed, except for rarely occurring events of negligible, random waiting time and verification time. We explore two situations. In the first case, Eve knows both Alice's and Bob's random noises. We show that, in this situation, Eve can quickly crack the secure key bit by using Ohm's Law. We also show that in this situation Eve can crack the secure key bit within a fraction of the bit exchange period even if her current and voltage measurements have only a single bit of resolution. In the other situation, Eve knows only Bob's random noise. Then Eve first can learn Bob's resistance value by using Ohm's Law. Therefore, she will have the same knowledge as Bob, thus at the end of the bit exchange period, she will know Alice's bit.

The second RNG attacks shown introduce and demonstrate two new statistical attacks against the Kirchhoff-Law-Johnson-Noise (KLJN) secure key exchange scheme. The attacks utilize compromised random number generators at Alice's/Bob's site(s). The case of partial correlations between Alice's/Bob's and Eve's probing noises is explored, that is, Eve’s knowledge of Alice’s and Bob’s noises is limited but not zero. We explore the bilateral situation where Eve has partial knowledge of Alice’s and Bob’s random number generators. It is shown that in this situation Eve can crack the secure key bit by taking the highest cross-correlation between her probing noises and the measured voltage noise in the wire. She can also crack the secure key bit by taking the highest cross-correlation between her noise voltages and her evaluation of Alice’s/Bob’s noise voltages. In the second attack, we explore the unilateral situation in which Eve has partial knowledge of only Alice’s random number generator thus only those noises (of Alice and Eve) are correlated. In this situation Eve can still crack the secure key bit, but for sufficiently low error probability, she needs to use the whole bit exchange period for the attack. The security of the KLJN key exchange scheme, similarly to other protocols, necessitates that the random number generator outputs are truly random for Eve.

The second focus topic of this thesis is the thermodynamical situation of the KLJN system. In all the original works, the proposed KLJN schemes required thermal equilibrium between the devices of the communicating parties to achieve perfect security. However, Vadai, et al, in (Nature) Science Reports 5 (2015) 13653 shows a modified scheme, where there is a non-zero thermal noise energy flow between the parties, yet the system seems to resist all the know attack types. We introduce a new attack type against their system. The new attack utilizes coincidence events between the line current and voltages. We show that there is non-zero information leak toward the Eavesdropper, even under idealized conditions. As soon as the thermal equilibrium is restored, the system becomes perfectly secure again. In conclusion, perfect unconditional security requires thermal equilibrium.

The final focus topic of this thesis is the nonlinear situation of the KLJN scheme. The attack is based on the nonlinearity of the noise generators. We explore the effect of total distortion ($\mathrm{TD}$) at the second order ($\mathrm{D}_2$), third order ($\mathrm{D}_3$), and a combination of the second and third orders ($\mathrm{D}_{2,3}$) on the security of the KLJN scheme. It is demonstrated that a   as little as 1\% results in a notable power flow along the information channel, which leads to a significant information leak. We also show that decreasing the effective temperature (that is, the wire voltage) and, in this way reducing nonlinearity, results in the KLJN scheme approaching perfect security.
 

\pagebreak{}


==> data/bibliography.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Fall 2016.
%
%  Author: Sean Zachary Roberson
%	 Version 3.16.09
%  Last updated 9/12/2016
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                           REFERENCES 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\phantomsection
\addcontentsline{toc}{chapter}{REFERENCES}

\renewcommand{\bibname}{{\normalsize\rm REFERENCES}}

%\bibliographystyle{ieeetr}
\bibliography{data/myReference}

==> data/conclusion.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Fall 2016.  
%
%
%  Author: Sean Zachary Roberson
%  Version 3.17.09
%  Last Updated: 9/21/2017
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                           SECTION I
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\chapter{\uppercase{Summary and Conclusions}\textsuperscript{1,2,4,5}}
\blfootnote{\textsuperscript{1}Part of this chapter is reprinted with permission from C.~Chamon, S.~Ferdous, and L.~B.~Kish, ``Deterministic random number generator attack against the Kirchhoff-law-Johnson-noise secure key exchange protocol," {\it Fluctuation and Noise Letters}, vol. 20, no. 5, 2021. Copyright 2021 by World Scientific Publishing Company.}
\blfootnote{\textsuperscript{2}Part of this chapter is reprinted with permission from C.~Chamon, S.~Ferdous, and L.~B.~Kish, ``Statistical random number generator attack against the Kirchhoff-law-Johnson-noise secure key exchange protocol," {\it Fluctuation and Noise Letters}, accepted for publication, 2021. Copyright 2021 by World Scientific Publishing Company.}
\blfootnote{\textsuperscript{4}Part of this chapter is reprinted with permission from C.~Chamon, L.~B.~Kish, ``Perspective--on the thermodynamics of perfect unconditional security," {\it Applied Physics Letters}, vol. 119, pp. 010501, 2021. Copyright 2021 by AIP Publishing.}
\blfootnote{\textsuperscript{5}Part of this chapter is reprinted with permission from C.~Chamon, S.~Ferdous, and L.~B.~Kish, ``Nonlinearity attack against the Kirchhoff-law-Johnson-noise secure key exchange protocol" {\it Fluctuation and Noise Letters}, in press, 2021. Copyright 2021 by World Scientific Publishing Company.}
\label{dissertation_conclusion}

Secure key exchange protocols utilize random numbers, and compromised random numbers lead to information leak. So far, it had been unknown how Eve can utilize full or partial knowledge about the random number generators to attack the KLJN protocol. To demonstrate how compromised RNGs can be utilized by Eve, we have introduced four deterministic RNG attacks and four statistical RNG attacks on the KLJN scheme.

For the deterministic attacks, we showed that if Eve knows the root of both Alice’s and Bob’s RNGs, that is, when she exactly knows the random numbers, she can use Ohm’s Law to crack the bit exchange. Eve can extract the bit very quickly, and she will learn the exchanged bit faster than Alice and Bob who know only their own random numbers. We showed that if Eve knows the seed of both Alice's and Bob's RNGs, that is, when she exactly knows the random numbers, she can crack the bit exchange even if her measurements have only one bit of resolution. The situation is similar to string verification in the noise-based logic systems. The cracking of the exchanged bit is exponentially fast; Eve can extract the bit within a fraction of the bit exchange period. Thus, Eve will learn the exchanged bit faster than Alice and Bob who know only their own random numbers.

We have also shown that if Eve knows the seed of only Alice’s RNG, she can still crack the secure bit by using Ohm's Law or a process of elimination. However, she is required to utilize the whole bit exchange period.

No statistical evaluation is needed, except for in the rarely-occurring event that Eve does not know which RNG belongs to which resistor, which will render in a waiting/verification (no-response) time that has a negligible effect on Eve’s cracking scheme.

For the statistical attacks, we explored various situations how RNGs compromised by statistical knowledge can be utilized by Eve. We have introduced four new attacks against the KLJN scheme. The defense against these attacks is the usage of true random number generators (with proper tamper resistance) at Alice's and Bob's sides. 

It is important to note that:
\begin{itemize}
\item To utilize these attacks, we implicitly used Kerckhoffs’s principle/Shannon's maxim \cite{Kerckhoffs}, which means Eve knows all the fine details of the protocol, including how the seeds are utilized and the RNG outputs timed.
\item This exploration was done assuming an ideal KLJN scheme. Future work would involve a practical circuit implementation or a cable simulator and related delays and transients.
\item Deterministic and statistical knowledge of the random number(s) by Eve is a strong security vulnerability. However, it is an illustrative way how such attacks can be developed.
\end{itemize}

We introduced a new passive attack that extracts information from the VMG-KLJN system and successfully compromises its security. On the other hand, the standard KLJN and the FCK1-VMG-KLJN schemes are immune against this attack because their net power flow is zero due to their thermal equilibrium feature. Our results prove that thermal equilibrium is essential for the perfect security of KLJN schemes, including their VMG-KLJN variations. Therefore, the Second Law of Thermodynamics is the fundamental component of the security of the VMG-KLJN system, too.

Nevertheless, we believe that, with careful design and proper compromises, the VMG-KLJN scheme \cite{VMGKLJN} has strong potential for applications in chip technology even if its security level is reduced compared to the features of original KLJN protocol. It is a security level that is sufficient for many practical applications but is reduced due to the deviation from the original KLJN. Its FCK1-VMG-KLN version \cite{FCKVMGKLJN} virtually eliminates the information leak, but then only three resistors can be freely chosen.

Finally, we introduced a new passive attack against the KLJN secure key exchange scheme when nonlinearity is present in the transfer function of the amplifier stage of noise generators. We demonstrated the effect of a 1\% total distortion at the second order ($\mathrm{D_2}$), third order ($\mathrm{D_3}$), and a combination of the two orders ($\mathrm{D_{2,3}}$) on the KLJN scheme.

We also demonstrated that, at a given nonlinear transfer characteristic, decreasing the effective voltage and, in this way reducing the nonlinearity, is a viable defense against the effect of nonlinearity in the KLJN scheme.

Our results showed that nonlinearity causes a notable power flow that leads to a significant information leak, so a careful design must be implemented such that the total distortion is kept at a minimum. 

Alternatively, privacy amplification protocols \cite{KLJN3,KLJN5,KLJN12,KLJN54} can also be used. For example, as an active privacy amplification, Alice and Bob can also measure and compare the power flow and discard a proper fraction of high-risk bits \cite{KLJN3,KLJN5}.

==> data/easybib.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Fall 2016.
%
%  Author: Sean Zachary Roberson
%	 Version 3.16.09
%  Last updated 9/12/2016
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                           REFERENCES 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\phantomsection
\addcontentsline{toc}{chapter}{REFERENCES}

\renewcommand{\bibname}{{\normalsize\rm REFERENCES}}

%\bibliographystyle{ieeetr}
\begin{thebibliography}{0}

%info theory

\bibitem{Shannon} C.~E.~Shannon, ``Communication theory of secrecy systems," {\it Bell Systems Technical Journal} pp. 656-715, 1949.

\bibitem{Kerckhoffs} Y.~Liang, H.~V.~Poor, S.~Shamai, ``Information theoretic security," {\it Foundations and Trends in Communications and Information Theory}, vol. 5, pp. 355-380, 2008.

%QKD

\bibitem{QKD1} H.P Yuen, ``Security of Quantum Key Distribution," {\it IEEE Access}, vol. 4, pp. 7403842, 2016.

\bibitem{QKD2} S.~Sajeed, A.~Huang, S.~Sun, F.~Xu, V.~Makarov, and M.~Curty, ``Insecurity of detector-device-independent quantum key distribution," \textit{Physical Review Letters}, vol. 117, no. 25, 2016.

\bibitem{QKD3} H.~P.~Yuen, ``Essential elements lacking in security proofs for quantum key distribution," \textit{Proc. SPIE}, vol. 8899, pp. 88990J–88990J-13, 2013.

\bibitem{QKD4} H.~P.~Yuen, ``Essential lack of security proof in quantum key distribution," arXiv preprint, https://arxiv.org/abs/1310.0842, 2013.

\bibitem{QKD5} O.~Hirota, ``Incompleteness and limit of quantum key distribution theory," arXiv preprint, https://arxiv.org/abs/1208.2106, 2012.

\bibitem{QKD6} N.~Jain, E.~Anisimova, I.~Khan, V.~Makarov, C.~Marquardt, and G.~Leuchs, Trojan-horse attacks threaten the security of practical quantum cryptography, \textit{New Journal of Physics}, vol. 16, 2014.

\bibitem{QKD7} I.~Gerhardt, Q.~Liu, A.~Lamas-Linares, J.~Skaar, C.~Kurtsiefer, and V.~Makarov, Full-field implementation of a perfect eavesdropper on a quantum cryptography system, \textit{Nature Communications}, vol. 2, no. 349, pp. 1-6, 2011.

\bibitem{QKD8} L.~Lydersen, C.~Wiechers, C.~Wittmann, D.~Elser, J.~Skaar, and V.~Makarov, Hacking commercial quantum cryptography systems by tailored bright illumination, \textit{Nature Photonics}, vol. 4, no. 10, pp. 686–689, 2010.

\bibitem{QKD9} I.~Gerhardt, Q.~Liu, A.~Lamas-Linares, J.~Skaar, V.~Scarani, V.~Makarov, and C.~Kurt-Siefer, ``Experimentally faking the violation of Bell’s inequalities," \textit{Physical Review Letters}, vol. 107, 2011.

\bibitem{QKD10} V.~Makarov and J.~Skaar, ``Fakes states attack using detector efficiency mismatch on SARG04, phase-time, DPSK, and Ekert Protocols," \textit{Quantum Information \& Computation}, vol. 8, no. 6, pp. 622–635, 2008.

\bibitem{QKD11} C.~Wiechers, L.~Lydersen, C.~Wittmann, D.~Elser, J.~Skaar, C.~Marquardt, V.~Makarov, and G.~Leuchs, ``After-gate attack on a quantum cryptosystem," \textit{New Journal of Physics}, vol. 13, 2011.

\bibitem{QKD12} L.~Lydersen, C.~Wiechers, C.~Wittmann, D.~Elser, J.~Skaar, and V.~Makarov, ``Thermal blinding of gated detectors in quantum cryptography, \textit{Optics Express}, vol. 18, no. 26, pp. 27938–27954, 2010.

\bibitem{QKD13} N.~Jain, C.~Wittmann, L.~Lydersen, C.~Wiechers, D.~Elser, C.~Marquardt, V.~Makarov, and G.~Leuchs, ``Device calibration impacts security of quantum key distribution," \textit{Physical Review Letters}, vol. 107, 2011.

\bibitem{QKD14} L.~Lydersen, J.~Skaar, and V.~Makarov, ``Tailored bright illumination attack on distributed-phase-reference protocols," \textit{Journal of Modern Optics}, vol. 58, no. 8, pp. 680–685, 2011.

\bibitem{QKD15} L.~Lydersen, M.~K.~Akhlaghi, A.~H.~Majedi, J.~Skaar, and V.~Makarov, ``Controlling a superconducting nanowire single-photon detector using tailored bright illumination," \textit{New Journal of Physics}, vol. 13, 2011.

\bibitem{QKD16} L.~Lydersen, V.~Makarov, and J.~Skaar, ``Comment on ``resilience of gated avalanche photodiodes against bright illumination attacks in quantum cryptography"," \textit{Applied Physics Letters}, vol. 98, 2011.

\bibitem{QKD17} P.~Chaiwongkhot, K.~B.~Kuntz, Y.~Zhang, A.~Huang, J.~P.~Bourgoin, S.~Sajeed, N.~Lütkenhaus, T.~Jennewein, and V.~Makarov, ``Eavesdropper's ability to attack a free-space quantum-key-distribution receiver in atmospheric turbulence," \textit{Physical Review A}, vol. 99, no. 6, 2019.

\bibitem{QKD18} G.~Gras, N.~Sultana, A.~Huang, T.~Jennewein, F.~Bussières, V.~Makarov, and H.~Zbinden, ``Optical control of single-photon negative-feedback avalanche diode detector," \textit{Journal of Applied Physics}, vol. 127, 2020.

\bibitem{QKD19} A.~Huang, R.~Li, V.~Egorov, S.~Tchouragoulov, K.~Kumar, and V.~Makarov, ``Laser-damage attack against optical attenuators in quantum key distribution," \textit{Physical Review Applied}, vol. 13, 2020.

\bibitem{QKD20} A.~Huang, \'{A}.~Navarrete, S.~H.~Sun, P.~Chaiwongkhot, M.~Curty, and V.~Makarov, ``Laser-seeding attack in quantum key distribution," \textit{Physical Review Applied}, vol. 12, 2019.

\bibitem{QKD21} V.~Chistiakov, A.~Huang, V.~Egorov, and V.~Makarov, ``Controlling single-photon detector ID210 with bright light," \textit{Optics Express}, vol. 27, no. 22, pp. 32253-32262 2019.

\bibitem{QKD22} A.~Fedorov, I.~Gerhardt, A.~Huang, J.~Jogenfors, Y.~Kurochkin, A.~Lamas-Linares, J.~\r{A}.~Larsson, G.~Leuchs, L.~Lydersen, V.~Makarov, and J.~Skaar, ``Comment on ``inherent security of phase coding quantum key distribution systems against detector blinding attacks"," \textit{Laser Physics Letters}, vol. 15, pp. 095203, 2018.

\bibitem{QKD23} A.~Huang, S.~Barz, E.~Andersson, and V.~Makarov, ``Implementation vulnerabilities in general quantum cryptography," \textit{New Journal of Physics}, vol. 20, pp. 103016, 2018.

\bibitem{QKD24} P.~V.~P.~Pinheiro, P.~Chaiwongkhot, S.~Sajeed, R.~T.~Horn, J.~P.~Bourgoin, T.~Jennewein, N.~L\"{u}tkenhaus, and V.~Makarov, ``Eavesdropping and countermeasures for backflash side channel in quantum cryptography," \textit{Optics Express}, vol. 26, pp. 21020, 2018. 

\bibitem{QKD25} A.~Huang, S.~H.~Sun, Z.~Liu, and V.~Makarov, ``Quantum key distribution with distinguishable decoy states," \textit{Physical Review A}, vol. 98, pp. 012330, 2018.

\bibitem{QKD26} H.~Qin, R.~Kumar, V.~Makarov, and R.~All\'{e}aume, ``Homodyne-detector-blinding attack in continuous-variable quantum key distribution," \textit{Physical Review A}, vol. 98, pp. 012312, 2018. 

\bibitem{QKD27} S.~Sajeed, C.~Minshull, N.~Jain, and V.~Makarov, Invisible Trojan-horse attack, \textit{Scientific Reports}, vol. 7, 2017.

\bibitem{QKD28} P.~Chaiwongkhot, S.~Sajeed, L.~Lydersen, and V.~Makarov, ``Finite-key-size effect in commercial plug-and-play QKD system," \textit{Quantum Science and Technology}, vol. 2, no. 4, pp. 044003, 2017. 

\bibitem{QKD29} A.~Huang, S.~Sajeed, P.~Chaiwongkhot, M.~Soucarros, M.~Legr\'{e}, and V.~Makarov, ``Testing random-detector-efficiency countermeasure in a commercial system reveals a breakable unrealistic assumption," \textit{IEEE Journal of Quantum Electronics}, vol. 52, no. 11, 2016.

\bibitem{QKD30} V.~Makarov, J.~P.~Bourgoin, P.~Chaiwongkhot, M.~Gagn\'{e}, T.~Jennewein, S.~Kaiser, R.~Kashyap, M.~Legr\'{e}, C.~Minshull, and S.~Sajeed, ``Creation of backdoors in quantum communications via laser damage," \textit{Physical Review A}, vol. 94, no. 3, 2016.

\bibitem{QKD31} S.~Sajeed, P.~Chaiwongkhot, J.~P.~Bourgoin, T.~Jennewein, N.~L\"{u}tkenhaus, and V.~Makarov, ``Security loophole in free-space quantum key distribution due to spatial-mode detector-efficiency mismatch," \textit{Physical Review A}, vol. 91, 2015.

\bibitem{QKD32} S.~Sajeed, I.~Radchenko, S.~Kaiser, J.~P.~Bourgoin, A.~Pappa, L.~Monat, M.~Legr\'{e}, and V.~Makarov, ``Attacks exploiting deviation of mean photon number in quantum key distribution and coin tossing," \textit{Physical Review A}, vol. 91, 2015.

\bibitem{QKD33} N.~Jain, B.~Stiller, I.~Khan, V.~Makarov, C.~Marquardt, and G.~Leuchs, ``Risk analysis of Trojan-horse attacks on practical quantum key distribution systems," \textit{IEEE Journal of Selected Topics in Quantum Electronics}, vol. 21, no. 3, pp. 168-177, 2015.

\bibitem{QKD34} N.~Jain, E.~Anisimova, I.~Khan, V.~Makarov, C.~Marquardt, and G.~Leuchs, ``Trojan-horse attacks threaten the security of practical quantum cryptography," \textit{New Journal of Physics}, vol. 16, 2014.

\bibitem{QKD35} M.~G.~Tanner, V.~Makarov, and R.~H.~Hadfield, ``Optimised quantum hacking of superconducting nanowire single-photon detectors," \textit{Optics Express}, vol. 22, pp. 6734, 2014. 

\bibitem{QKD36} A.~N.~Bugge, S.~Sauge, A.~M.~M.~Ghazali, J.~Skaar, L.~Lydersen, and V.~Makarov, ``Laser damage helps the eavesdropper in quantum cryptography," \textit{Physical Review Letters}, vol. 112, no. 7, 2014.

\bibitem{QKD37} Q.~Liu, A.~Lamas-Linares, C.~Kurtsiefer, J.~Skaar, V.~Makarov, and I.~Gerhardt, ``A universal setup for active control of a single-photon detector," \textit{The Review of Scientific Instruments}, vol. 85, pp. 013108, 2014.

%KLJN

\bibitem{APL} C.~Chamon, L.~B.~Kish, ``Perspective--on the thermodynamics of perfect unconditional security," {\it Applied Physics Letters}, vol. 119, pp. 010501, 2021.

\bibitem{RNG} C. Chamon, S. Ferdous, and L.B. Kish, ``Random number generator attack against the Kirchhoff-law-Johnson-noise secure key exchange protocol," arXiv preprint, https://arxiv.org/abs/2005.10429, 2020.

\bibitem{deterministicRNG} C.~Chamon, S.~Ferdous, and L.~B.~Kish, ``Deterministic random number generator attack against the Kirchhoff-law-Johnson-noise secure key exchange protocol," {\it Fluctuation and Noise Letters}, vol. 20, no. 5, 2021.

\bibitem{statisticalRNG} C.~Chamon, S.~Ferdous, and L.~B.~Kish, ``Statistical random number generator attack against the Kirchhoff-law-Johnson-noise secure key exchange protocol," {\it Fluctuation and Noise Letters}, accepted for publication, 2021.

\bibitem{nonlinearity} C.~Chamon, S.~Ferdous, and L.~B.~Kish, ``Nonlinearity attack against the Kirchhoff-law-Johnson-noise secure key exchange protocol,"  {\it Fluctuation and Noise Letters}, in press, 2021.

\bibitem{KLJNbook} L.~B.~Kish, The Kish Cypher: The Story of KLJN for Unconditional Security, New Jersey: World Scientific, 2017.

\bibitem{KLJN1} L.~B.~Kish, ``Totally secure classical communication utilizing Johnson (-like) noise and Kirchhoff's law," \textit{Physics Letters A}, vol. 352, no. 3, pp. 178-182, 2006.

\bibitem{KLJN2} A.~Cho, ``Simple noise may stymie spies without quantum weirdness," \textit{Science}, vol. 309, no. 5744, pp. 2148, 2005.

\bibitem{KLJN3} L.~B.~Kish and C.~G.~Granqvist, ``On the security of the Kirchhoff-law-Johnson-noise (KLJN) communicator," \textit{Quantum Information Processing}, vol. 13, no. 10, pp. 2213-2219, 2014.

\bibitem{KLJN4} L.~B.~Kish, ``Enhanced secure key exchange systems based on the Johnson-noise scheme," \textit{Metrology and Measurement Systems}, vol. 20, no. 10, pp. 191-204, 2013.

\bibitem{KLJN5} L.~B.~Kish and T.~Horvath, ``Notes on recent approaches concerning the Kirchhoff-law–Johnson-noise based secure key exchange," \textit{Physics Letters A}, vol. 373, pp. 2858-2868, 2009.

\bibitem{VMGKLJN} G.~Vadai, R.~Mingesz, and Z.~Gingl, ``Generalized Kirchhoff-law-Johnson-noise (KLJN) secure key exchange system using arbitrary resistors," \textit{Scientific Reports}, vol. 5, 2015.

\bibitem{FCKVMGKLJN} S.~Ferdous, C.~Chamon, and L.~B.~Kish, ``Comments on the ``generalized" KJLN key exchanger with arbitrary resistors: power, impedance, security," \textit{Fluctuation and Noise Letters}, vol. 20, pp. 2130002, 2020.

\bibitem{KLJN8} L.~B.~Kish and C.~G.~Granqvist, ``Random-resistor-random-temperature Kirchhoff-law-Johnson-noise(RRRT -KLJN) key exchange," \textit{Metrology and Measurement Systems}, vol. 23, pp. 3-11, 2016.

\bibitem{KLJN9} J.~Smulko, ``Performance analysis of the ‘intelligent’Kirchhoff’s-law–Johnson-noise secure key exchange," \textit{Fluctuations and Noise Letters}, vol. 13, pp. 1450024, 2014.

\bibitem{KLJN10} R.~Mingesz, Z.~Gingl, and L.~B.~Kish, ``Johnson(-like)-noise-Kirchhoff-loop based secure classical communicator characteristics, for ranges of two to two thousand kilometers, via model-line," \textit{Physics Letters A}, vol. 372, pp. 978–984, 2008.

\bibitem{KLJN11} R.~Mingesz, L.~B.~Kish, Z.~Gingl, C.~G.~Granqvist, H.~Wen, F.~Peper, T.~Eubanks, and G.~Schmera, ``Unconditional security by the laws of classical physics," \textit{Metrology and Measurement Systems}, vol. 20, pp. 3–16, 2013.

\bibitem{KLJN12} T.~Horvath, L.~B.~Kish, and J.~Scheuer, ``Effective privacy amplification for secure classical communications," \textit{EPL}, vol. 94, pp. 28002, 2011.

\bibitem{KLJN13} Y.~Saez and L.~B.~Kish, ``Errors and their mitigation at the Kirchhoff-law-Johnson-noise secure key exchange," \textit{PLoS ONE}, vol. 8, no. 11, 2013.

\bibitem{GaussianVMG} R.~Mingesz, G.~Vadai, and Z.~Gingl, ``What kind of noise guarantees security for the Kirchhoff-loop-Johnson-noise key exchange?" \textit{Fluctuation and Noise Letters}, vol. 13, no. 3, pp. 1450021, 2014.

\bibitem{KLJN15} Y.~Saez, L.~B.~Kish, R.~Mingesz, Z.~Gingl, and C.~G.~Granqvist, ``Current and voltage based bit errors and their combined mitigation for the Kirchhoff-law-Johnson-noise secure key exchange," \textit{Journal of Computational Electronics}, vol. 13, pp. 271–277, 2014.

\bibitem{KLJN16} Y.~Saez, L.~B.~Kish, R.~Mingesz, Z.~Gingl, and C.~G.~Granqvist, ``Bit errors in the Kirchhoff-law-Johnson-noise secure key exchange," \textit{International Journal of Modern Physics: Conference Series}, vol. 33, pp. 1460367, 2014.

\bibitem{KLJN17} Z.~Gingl and R.~Mingesz, ``Noise properties in the ideal Kirchhoff-law-Johnson-noise secure communication system," \textit{PLoS ONE}, vol. 9, no. 4, 2014.

\bibitem{KLJN18} P.~L.~Liu, ``A key agreement protocol using band-limited random signals and feedback," \textit{IEEE Journal of Lightwave Technology}, vol. 27, no. 23, pp. 5230-5234, 2009.

\bibitem{KLJN19} L.~B.~Kish and R.~Mingesz, ``Totally secure classical networks with multipoint telecloning (teleportation) of classical bits through loops with Johnson-like noise," \textit{Fluctuation and Noise Letters}, vol. 6, no. 2, pp. C9–C21, 2006.

\bibitem{KLJN20} L.~B.~Kish, ``Methods of using existing wire lines (power lines, phone lines, internet lines) for totally secure classical communication utilizing Kirchoff's law and Johnson-like noise," arXiv preprint, https://arxiv.org/abs/physics/0610014, 2006.

\bibitem{KLJN21} L.~B.~Kish and F.~Peper, ``Information networks secured by the laws of physics," \textit{IEICE Transactions on the Fundamentals of Communications, Electronics, Information, and Systems}, vol. E95–B, no. 5, pp. 1501-1507, 2012.

\bibitem{KLJN22} E.~Gonzalez, L.~B.~Kish, R.~S.~Balog, and P.~Enjeti, ``Information theoretically secure, enhanced Johnson noise based key distribution over the smart grid with switched filters," \textit{PloS One}, vol. 8, no. 7, 2013.

\bibitem{KLJN23} E.~Gonzalez, L.~B.~Kish, and R.~Balog, ``Encryption Key Distribution System and Method," U.S. Patent \#US9270448B2 , https://patents.google.com/patent/US9270448B2, 2016.

\bibitem{KLJN24} E.~Gonzalez, R.~Balog, R.~Mingesz, and L.~B.~Kish, ``Unconditional security for the smart power grids and star networks," \textit{23rd International Conference on Noise and Fluctuations (ICNF 2015)}, Xian, China, June 2-5, 2015.

\bibitem{KLJN25} E.~Gonzalez, R.~S.~Balog, and L.~B.~Kish, ``Resource requirements and speed versus geometry of unconditionally secure physical key exchanges," \textit{Entropy}, vol. 17, no. 4, pp. 2010–2014, 2015.

\bibitem{KLJN26} E.~Gonzalez and L.~B.~Kish, ``Key exchange trust evaluation in peer-to-peer sensor networks with unconditionally secure key exchange," \textit{Fluctuation and Noise Letters}, vol. 15, pp. 1650008, 2016.

\bibitem{KLJN27} L.~B.~Kish and O.~Saidi, ``Unconditionally secure computers, algorithms and hardware, such as memories, processors, keyboards, flash and hard drives," \textit{Fluctuation and Noise Letters}, vol. 8, pp. L95–L98, 2008.

\bibitem{KLJN28} L.~B.~Kish, K.~Entesari, C.~G.~Granqvist, and C.~Kwan, ``Unconditionally secure credit/debit card chip scheme and physical unclonable function," \textit{Fluctuation and Noise Letters}, vol. 16, pp. 1750002, 2017.

\bibitem{KLJN29} L.~B.~Kish and C.~Kwan, ``Physical unclonable function hardware keys utilizing Kirchhoff-law-Johnson noise secure key exchange and noise-based logic," \textit{Fluctuation and Noise Letters}, vol. 12, pp. 1350018, 2013. 

\bibitem{KLJN30} Y.~Saez, X.~Cao, L.~B.~Kish, and G.~Pesti, ``Securing vehicle communication systems by the KLJN key exchange protocol," \textit{Fluctuation and Noise Letters}, vol. 13, pp. 1450020, 2014.

\bibitem{KLJN31} X.~Cao, Y.~Saez, G.~Pesti, and L.~B.~Kish, ``On KLJN-based secure key distribution in vehicular communication networks," \textit{Fluctuation and Noise Letters}, vol. 14, pp. 1550008, 2015. 

\bibitem{KLJN32} L.~B.~Kish and C.~G.~Granqvist, ``Enhanced usage of keys obtained by physical, unconditionally secure distributions," \textit{Fluctuation and Noise Letters}, vol. 14, pp. 1550007, 2015.

\bibitem{KLJN33} P.~L.~Liu, ``A complete circuit model for the key distribution system using resistors and noise sources," \textit{Fluctuation and Noise Letters}, vol. 19, pp. 2050012, 2020.

\bibitem{KLJN34} M.~Y.~Melhem and L.~B.~Kish, ``Generalized DC loop current attack against the KLJN secure key exchange scheme," \textit{Metrology and Measurement Systems}, vol. 26, pp. 607-616, 2019.

\bibitem{KLJN35} M.~Y.~Melhem and L.~B.~Kish, ``A static-loop-current attack against the Kirchhoff-law-Johnson-noise (KLJN) secure key exchange system," \textit{Applied Sciences}, vol. 9, pp. 666, 2019.

\bibitem{KLJN36} M.~Y.~Melhem and L.~B.~Kish, ``The problem of information leak due to parasitic loop currents and voltages in the KLJN secure key exchange scheme," \textit{Metrology and Measurement Systems}, vol. 26, pp. 37-40, 2019.

\bibitem{KLJN37} M.~Y.~Melhem and L.~B.~Kish, ``Man in the middle and current injection attacks against the KLJN key exchanger compromised by DC sources," {\it Fluctuation and Noise Letters}, vol. 20, no. 2, pp. 2150011, 2021.

\bibitem{KLJN38} M.~Y.~Melhem, C.~Chamon, S.~Ferdous, L.~B.~Kish, ``Alternating (AC) Loop Current Attacks against the KLJN Secure Key Exchange Scheme," {\it Fluctuation and Noise Letters}, 2021.

\bibitem{KLJN39} P.~L.~Liu, ``Re-examination of the cable capacitance in the key distribution system using resistors and noise sources," \textit{Fluctuation and Noise Letters}, vol. 16, pp. 1750025, 2017.

\bibitem{KLJN40} H.~P.~Chen, M.~Mohammad, and L.~B.~Kish, ``Current injection attack against the KLJN secure key exchange," \textit{Metrology and Measurement Systems}, vol. 23, pp. 173-181, 2016.

\bibitem{KLJN41} G.~Vadai, Z.~Gingl, and R.~Mingesz, ``Generalized attack protection in the Kirchhoff-law-Johnson-noise key exchanger," \textit{IEEE Access}, vol. 4, pp. 1141-1147, 2016.

\bibitem{KLJN42} H.~P.~Chen, E.~Gonzalez, Y.~Saez, and L.~B.~Kish, ``Cable capacitance attack against the KLJN secure key exchange," \textit{Information}, vol. 6, pp. 719-732, 2015.

\bibitem{KLJN43} L.~B.~Kish and C.~G.~Granqvist, ``Elimination of a second-law-attack, and all cable-resistance-based attacks, in the Kirchhoff-law-Johnson-noise (KLJN) secure key exchange system," \textit{Entropy}, vol. 16, pp. 5223-5231, 2014.

\bibitem{KLJN44} L.~B.~Kish and J.~Scheuer, ``Noise in the wire: the real impact of wire resistance for the Johnson (-like) noise based secure communicator," \textit{Physics Letters A}, vol. 374, pp. 2140-2142, 2010.

\bibitem{KLJN45} F.~Hao, ``Kish's key exchange scheme is insecure," \textit{IEE Proceedings - Information Security}, vol. 153, no. 4, pp. 141-142, 2006.

\bibitem{KLJN46} L.~B.~Kish, Response to Feng Hao's paper ``Kish's key exchange scheme is insecure," \textit{Fluctuation and Noise Letters}, vol. 6, pp. C37-C41, 2006.

\bibitem{KLJN47} L.~B.~Kish, ``Protection against the man-in-the-middle-attack for the Kirchhoff-loop-Johnson (-like)-noise cipher and expansion by voltage-based security," \textit{Fluctuation and Noise Letters}, vol. 6, pp. L57-L63, 2006.

\bibitem{KLJN48} L.~J.~Gunn, A.~Allison, and D.~Abbott, ``A new transient attack on the Kish key distribution system," \textit{IEEE Access}, vol. 3, pp. 1640-1648, 2015.

\bibitem{KLJN49} L.~B.~Kish and C.~G.~Granqvist, ``Comments on ``a new transient attack on the Kish key distribution system"," \textit{Metrology and Measurement Systems}, vol. 23, pp. 321-331, 2015.

\bibitem{KLJN50} L.~J.~Gunn, A.~Allison, and D.~Abbott, ``A directional wave measurement attack against the Kish key distribution system," \textit{Scientific Reports}, vol. 4, pp. 6461, 2014.

\bibitem{KLJN51} H.~P.~Chen, L.~B.~Kish, and C.~G.~Granqvist, ``On the ``cracking" scheme in the paper ``a directional coupler attack against the Kish key distribution system" by Gunn, Allison and Abbott," \textit{Metrology and Measurement Systems}, vol. 21, pp. 389-400, 2014.

\bibitem{KLJN52} H.~P.~Chen, L.~B.~Kish, C.~G.~Granqvist, and G.~Schmera, ``Do electromagnetic waves exist in a short cable at low frequencies? What does physics say?" \textit{Fluctuation and Noise Letters}, vol. 13, pp. 1450016, 2014.

\bibitem{KLJN53} L.~B.~Kish, Z.~Gingl, R.~Mingesz, G.~Vadai, J.~Smulko, and C.~G.~Granqvist, ``Analysis of an attenuator artifact in an experimental attack by Gunn–Allison–Abbott against the Kirchhoff-law–Johnson-noise (KLJN) secure key exchange system," \textit{Fluctuation and Noise Letters}, vol. 14, pp. 1550011, 2015.                                                     

\bibitem{KLJN54} L.~B.~Kish, D.~Abbott, and C.~G.~Granqvist, ``Critical analysis of the Bennett–Riedel attack on secure cryptographic key distributions via the Kirchhoff-law–Johnson-noise scheme," \textit{PloS One}, vol. 8, no. 12, 2013.

%RNG PAPERS

\bibitem{RNG1} R.~Halprin and M.~Naor, Games for extracting randomness, \textit{Proc. SOUPS}, New York, NY, USA, 2009.

\bibitem{RNG2} J.~Kelsey, B.~Schneier, D.~Wagner, and C.~Hall, ``Cryptanalytic attacks on pseudorandom number generators," \textit{Fast Software Encryption}, Springer-Verlag Berlin Heidelberg, vol. 1372, pp. 168–188, 1998.

\bibitem{RNG3} I.~Goldberg and D.~Wagner, ``Randomness and netscape browser," \textit{Dr. Dobb's Journal}, 1996.

\bibitem{RNG4} L.~Dorrendorf, Z.~Gutterman, and B.~Pinkas, ``Cryptanalysis of the Windows random number generator," \textit{Proc. CCS}, New York, NY, USA, 2007. 

\bibitem{RNG5} E.~Barker and J.~Kelsey, \textit{Recommendation for random number generation using deterministic random bit generators}, Gaithersburg, MD, USA: NIST (2012).

\bibitem{RNG6} K.~Nohl, D.~Evans, S.~Starbug, and H.~Pl\"{o}tz, ``Reverse-engineering a cryptographic RFID tag," \textit{Proc. SS}, San Jose, CA, USA, 2008.

%OTHER

\bibitem{NBL} L.~Kish, S.~Khatri, and T.~Horvath, ``Computation using noise-based logic: efficient string verification over a slow communication channel," \textit{The European Physical Journal B}, vol. 79, pp. 85–90, 2011.

\bibitem{Razavi} B.~Razavi, RF Microelectronics, Prentice Hall, 2011.
\end{thebibliography}

==> data/intro.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Fall 2016.  
%
%
%  Author: Sean Zachary Roberson
%  Version 3.17.09
%  Last Updated: 9/21/2017
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                           SECTION I
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\pagestyle{plain} % No headers, just page numbers
\pagenumbering{arabic} % Arabic numerals
\setcounter{page}{1}


\chapter{\uppercase {Introduction}\textsuperscript{1,2}}
\blfootnote{\textsuperscript{1}Part of this chapter is reprinted with permission from C.~Chamon, S.~Ferdous, and L.~B.~Kish, ``Deterministic random number generator attack against the Kirchhoff-law-Johnson-noise secure key exchange protocol," {\it Fluctuation and Noise Letters}, vol. 20, no. 5, 2021. Copyright 2021 by World Scientific Publishing Company.}
\blfootnote{\textsuperscript{2}Part of this chapter is reprinted with permission from C.~Chamon, S.~Ferdous, and L.~B.~Kish, ``Statistical random number generator attack against the Kirchhoff-law-Johnson-noise secure key exchange protocol," {\it Fluctuation and Noise Letters}, accepted for publication, 2021. Copyright 2021 by World Scientific Publishing Company.}
\label{dissertation_intro}

\section{On Secure Communications}
%What is the topic of the paper? Why should I as a reader care about that topic? What has been done previously? What is the novelty that this paper brings to the table?
One way to establish the security of a communication is through encryption, that is, the conversion of plaintext into ciphertext via a cipher \cite{Shannon}. Figure~\ref{symmetric} provides the general scope of symmetric-key cryptography \cite{Shannon}. The key is a string of random bits and both communicating parties Alice and Bob use the same key and ciphers to encrypt and decrypt their plaintext.

\begin{figure}[ht!]
	\centering
	\includegraphics[width=6in]{symmetric.pdf}
	\caption{Symmetric-key cryptography \cite{Shannon}. Alice and Bob securely exchange a key (a string of random bits) through an information channel. The ciphers encrypt plaintext into the ciphertext $C$. The secure key is $K$, the plaintext messages of Alice and Bob are denoted by $P_\mathrm{A}$ and $P_\mathrm{B}$, respectively, and the ciphertext is a function $C$($P$,$K$).}
\label{symmetric}
\end{figure}

For a plaintext message $P$ and a secure key $K$, the encrypted message, or the ciphertext $C$, is a function of $P$ and $K$, that is,

\begin{equation}
C=C(P,K).\label{ciphertext}
\end{equation}

\noindent In symmetric-key cryptography, for decryption, the inverse operation is used:

\begin{equation}
P=C^{-1}[C(P,K),K].\label{plaintext}
\end{equation}

\noindent Because the secure keys must be the same at the two sides (shared secret), another type of secure data exchange is needed before the encryption can begin: the secure key exchange, which is the generation and distribution of the secure key over the communication channel. Usually, this is the most demanding process in the secure communication because the communication channel is accessible by Eve, thus the secure key exchange is itself a secure communication where the cipher scheme shown in Figure~\ref{symmetric} cannot be used. Eve records the whole communication during the key exchange, too. She knows every detail of the devices, protocols, and algorithms in the permanent communication system (as stated by Kerckhoffs's\textsuperscript{3} principle/Shannon’s maxim \cite{Kerckhoffs}), except for the key. In the ideal case of perfect security, the key is securely generated/shared, immediately used by a One Time Pad \cite{QKD1}, and discarded after the usage. In practical cases, usually there are deviations from these strict conditions, yet the general rule holds: a secure system cannot be more secure than its key.

\blfootnote{\textsuperscript{3}Auguste Kerckhoffs, not to be confused with Gustav Kirchhoff.}

Our focus topic is the unconditionally secure Kirchhoff-law-Johnson-noise (KLJN) symmetric-key exchanger.

\section{The KLJN Scheme}
\label{KLJN}
The KLJN system \cite{APL,RNG,deterministicRNG,statisticalRNG,nonlinearity,KLJNbook,KLJN1,KLJN2,KLJN3,KLJN4,KLJN5,VMGKLJN,FCKVMGKLJN,KLJN8,KLJN9,KLJN10,KLJN11,KLJN12,KLJN13,GaussianVMG,KLJN15,KLJN16,KLJN17,KLJN18,KLJN19,KLJN20,KLJN21,KLJN22,KLJN23,KLJN24,KLJN25,KLJN26,KLJN27,KLJN28,KLJN29,KLJN30,KLJN31,KLJN32,KLJN33,KLJN34,KLJN35,KLJN36,KLJN37,KLJN38,KLJN39,KLJN40,KLJN41,KLJN42,KLJN43,KLJN44,KLJN45,KLJN46,KLJN47,KLJN48,KLJN49,KLJN50,KLJN51,KLJN52,KLJN53,KLJN54} is a statistical physical scheme based on the Second Law of Thermodynamics. It is a classical (statistical) physical alternative of Quantum Key Distribution (QKD), the base of quantum cryptography, which utilizes quantum physical photonic features.

As an illustration of the difficulties and depth of the issues of security, in papers \cite{QKD1,QKD2,QKD3,QKD4,QKD5,QKD6,QKD7,QKD8,QKD9,QKD10,QKD11,QKD12,QKD13,QKD14,QKD15,QKD16,QKD17,QKD18,QKD19,QKD20,QKD21,QKD22,QKD23,QKD24,QKD25,QKD26,QKD27,QKD28,QKD29,QKD30,QKD31,QKD32,QKD33,QKD34,QKD35,QKD36,QKD37}, important criticisms and attacks are presented about QKD indicating some of the most important aspects of unconditionally secure quantum hardware and their theory. Very recently, National Security Agency (NSA) has made a public statement: "NSA does not recommend the usage of quantum key distribution and quantum cryptography for securing the transmission of data in National Security Systems (NSS)...". While we have reservations about this NSA statement, it inherently brings KLJN up for further considerations. Both the QKD and KLJN schemes count as "Post-Quantum" hardware solutions because they are resilient against any (past and future) computing schemes, including quantum computers, but only the KLJN scheme can be integrated on chips with currently available technology to offer unconditional security of communication within computers and instruments.

Figure~\ref{figKLJN} illustrates the core of the KLJN scheme. The two communicating parties Alice and Bob are connected via a wire. They have identical pairs of resistors $R_\mathrm{A}$ and $R_\mathrm{B}$. The statistically independent thermal noise voltages $U_\mathrm{H,A}(t)$, $U_\mathrm{L,A}(t)$, and $U_\mathrm{H,B}(t)$, $U_\mathrm{L,B}(t)$ represent the noise voltages of the resistors $R_\mathrm{H}$ and $R_\mathrm{L}$ ($R_\mathrm{H} > R_\mathrm{L}$) of Alice and Bob, respectively, which are generated from random number generators (RNGs) and must have a Gaussian amplitude distribution \cite{GaussianVMG,KLJN17}.

\begin{figure}[ht!]
	\centering
	\includegraphics[width=6in]{figKLJN.pdf}
\caption{The core of the KLJN scheme. The two communicating parties Alice and Bob are connected via a wire. The wire voltage and current are denoted as $U_\mathrm{w}(t)$ and $I_\mathrm{w}(t)$, respectively. The parties have identical pairs of resistors $R_\mathrm{H}$ and $R_\mathrm{L}$ ($R_\mathrm{H} > R_\mathrm{L}$) that are randomly selected and connected to the wire at the beginning of the bit exchange period. The statistically independent thermal noise voltages $U_\mathrm{H,A}(t)$, $U_\mathrm{L,A}(t)$, and $U_\mathrm{H,B}(t)$, $U_\mathrm{L,B}(t)$ represent the noise voltages of the resistors $R_\mathrm{H}$ and $R_\mathrm{L}$ of Alice and Bob, respectively.}
\label{figKLJN}
\end{figure}

At the beginning of each bit exchange period (BEP), Alice and Bob randomly choose one of their resistors to connect to the wire. The wire voltage $U_\mathrm{w}(t)$ and current $I_\mathrm{w}(t)$ are as follows:

\begin{equation}
U_\mathrm{w}(t)=I_\mathrm{w}(t)R_\mathrm{B}+U_\mathrm{B}(t),\label{Uw}
\end{equation}

\begin{equation}
I_\mathrm{w}(t)=\frac{U_\mathrm{A}(t)-U_\mathrm{B}(t)}{R_\mathrm{A}+R_\mathrm{B}}\label{Iw}
\end{equation}

\noindent where $U_\mathrm{A}(t)$ and $U_\mathrm{B}(t)$ denote the instantaneous noise voltage of the resistor chosen by Alice and Bob, respectively. Alice and Bob (as well as Eve) use the mean-square voltage of the wire to assess the situation. According to the Johnson formula,

\begin{equation}
U_{\mathrm{w,eff}}^2=4kT_{\mathrm{eff}}R_{\mathrm{p}}\Delta{f_{\mathrm{B}}},\label{meansquare}
\end{equation}

\noindent where $k$ is the Boltzmann constant (1.38 x 10\textsuperscript{-23}~J/K), $T_\mathrm{eff}$ is the publicly agreed effective temperature, $R_\mathrm{P}$ is the parallel combination of Alice and Bob’s chosen resistors, given by

\begin{equation}
R_{\mathrm{P}}=\frac{R_{\mathrm{A}}R_\mathrm{B}}{R_\mathrm{A}+R_\mathrm{B}},\label{Rp}
\end{equation}

\noindent and $\Delta$$f_\mathrm{B}$ is the noise bandwidth of the generators.

Four possible resistance situations can be formed by Alice and Bob: HH, LL, LH, and HL. Using the Johnson formula, these correspond to three mean-square voltage levels, as shown in Figure~\ref{threelevels}. 

\begin{figure}[ht!]
\centering
	\includegraphics[width=6in]{three_levels.pdf}
\caption{The three mean-square voltage levels. The HH and LL cases represent insecure situations because they form distinct mean-square voltages. The HL and LH cases represent secure bit exchange because Eve cannot distinguish between the corresponding two resistance situations (HL and LH). On the other hand, Alice and Bob can determine the resistance at the other end because they know their own connected resistance values.}
\label{threelevels}
\end{figure}

The HH and LL cases represent insecure situations because they form distinct mean-square voltages. The HL and LH cases represent secure bit exchange because Eve cannot distinguish between the corresponding two resistance situations (HL and LH). On the other hand, Alice and Bob can determine the resistance at the other end because they know their own connected resistance values.

Several attacks against the KLJN system have been proposed \cite{APL,RNG,deterministicRNG,statisticalRNG,nonlinearity,KLJN34,KLJN35,KLJN36,KLJN37,KLJN38,KLJN39,KLJN40,KLJN41,KLJN42,KLJN43,KLJN44,KLJN45,KLJN46,KLJN47,KLJN48,KLJN49,KLJN50,KLJN51,KLJN52,KLJN53,KLJN54}, but no attack has been able to compromise its information-theoretic (unconditional) security because each known attack is either invalid (conceptually incorrect errors in theory and/or experiments) or can be nullified by a corresponding defense scheme such that Eve’s information entropy about the key approaches the bit length of the key, while Alice’s and Bob’s information entropy about the key approaches zero. 

The rest of this dissertation is as follows. Chapter~\ref{RNG_chapter} introduces four deterministic and four statistical attacks based on the assumption that the random number generators Alice and Bob use to generate their noises are compromised. Chapter~\ref{ZCA_chapter} introduces an attack based on coincidence events between the wire voltage and current. Chapter~\ref{nonlinearity_chapter} introduces an attack based on the nonlinearity of Alice's and Bob's noise generators. Finally, Chapter~\ref{dissertation_conclusion} summarizes and concludes this dissertation.

==> data/section1a.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Fall 2016.  
%
%
%  Author: Sean Zachary Roberson
%  Version 3.17.09
%  Last Updated: 9/21/2017
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                           SECTION I
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\pagestyle{plain} % No headers, just page numbers
\pagenumbering{arabic} % Arabic numerals
\setcounter{page}{1}


\chapter{\uppercase {Random Number Generator Attack against the Kirchhoff-Law-Johnson-Noise Secure Key Exchanger}}

\section{Background}

\subsection{Random Number Generator Attacks}
\label{RNG}
There are two classes of practical random number generators: true (physical) and computational. The nature of computational RNGs is that they collect randomness from various low-entropy input streams and try to generate outputs that are in practice indistinguishable from truly random streams \cite{RNG1,RNG2,RNG3,RNG4,RNG5,RNG6}. The randomness of an RNG relies on the uncertainty of the random seed, or initialization vector, and a long sequence with uniform distribution. The moment an adversary learns the seed, the outputs are known, and the RNG is compromised.

Various RNG attacks exist against conditionally secure communications \cite{RNG1,RNG2,RNG3,RNG4,RNG5,RNG6}. Unconditionally secure communications also require true random numbers for perfect security, and that is also true for the noises of Alice and Bob and for the randomness of their switch-driving, which uses a different RNG from the voltage sources. However, it is unclear how Eve can utilize compromised RNGs, from which she has obtained by spying on the root of the RNGs, to attack the KLJN scheme. The RNG outputs must imitate thermal noise, and in many practical applications, only a computational RNG is possible. Here, we demonstrate with two simple attack examples that compromised noises lead to information leak.

The rest of this paper is organized as follows. Section~\ref{experiment} describes two new attack protocols and the waiting/verification (no-response) time scenario, and Section~\ref{conclusion} concludes this paper.

\section{Attack Methodology}
\label{experiment}

Two theoretical situations are introduced where Eve can use compromised RNGs to crack the KLJN scheme: one where Eve knows the roots of both Alice’s and Bob’s generators (bilateral parameter knowledge), and another where Eve knows the root of only Bob's generator (unilateral parameter knowledge). A scenario is also introduced where the only statistical evaluation needed is in the rarely-occurring event of a negligible waiting/verification (no-response) time.

\subsection{Bilateral Parameter Knowledge}
\label{bilateral}
Eve knows the roots of both Alice’s and Bob’s RNGs, thus she knows the instantaneous amplitudes of the noise voltage generators for each of their resistors (see Fig.~\ref{figKLJN}). With $U_{\mathrm{H,A}}(t)$, $U_{\mathrm{L,A}}(t)$, $U_{\mathrm{H,B}}(t)$, and $U_{\mathrm{L,B}}(t)$ known, Eve measures the wire voltage $U_{\mathrm{w}}(t)$ and the wire current  $I_{\mathrm{w}}(t)$ to determine $R_{\mathrm{B}}$ (see Eq.~\eqref{Uw}) and determines that the correct waveform for $R_{\mathrm{B}}$ is a flat line at the expected resistor value, while the incorrect waveform is a noise with divergent spikes. This is because the difference between $U_{\mathrm{w}}(t)$ and $U_{\mathrm{B}}(t)$ is directly proportional to $I_{\mathrm{w}}(t)$, with $R_{\mathrm{B}}$ as the scaling factor, and the incorrect noise voltage for $U_{\mathrm{B}}(t)$ would not render a constant value for $R_{\mathrm{B}}$.

A realization of the waveforms for $R_{\mathrm{B}}$ is shown in Fig.~\ref{RB} at $R_{\mathrm{H}} = 100$~k\textOmega, $R_{\mathrm{L}} = 10$~k\textOmega, $T_{\mathrm{eff}} = 10^{18}$~K, and $\Delta f_{\mathrm{B}} = 500$~Hz. At the present situation, the flat line corresponds to $R_{\mathrm{H}}$, thus Eve determines that Bob has chosen $R_{\mathrm{H}}$. With $U_{\mathrm{A}}(t)$, $U_{\mathrm{B}}(t)$, $R_{\mathrm{B}}$, and $I_{\mathrm{w}}(t)$ known, Eve uses Eq.~\eqref{Iw} to solve for $R_{\mathrm{A}}$.

\begin{figure}[ht!]
\centering
	\includegraphics[width=4.25in]{resistor_waveform.pdf}
\caption{\ A realization of the waveforms for $R_{\mathrm{B}}$ (see Eq.~\eqref{Uw}) at $R_{\mathrm{H}} = 100$~k\textOmega, $R_{\mathrm{L}} = 10$~k\textOmega, $T_{\mathrm{eff}} = 10^{18}$~K, and $\Delta f_{\mathrm{B}} = 500$~Hz. The flat line corresponds to $R_{\mathrm{H}}$, thus Eve determines that Bob has chosen $R_{\mathrm{H}}$. The incorrect waveform is a noise with divergent spikes.}
\label{RB}
\end{figure}

\subsection{Unilateral Parameter Knowledge}
\label{unilateral}
Eve knows only the root of Bob's generator RNG, thus she knows merely the noise generator outputs of Bob's resistors, $U_{\mathrm{L,B}}(t)$ and $U_{\mathrm{H,B}}(t)$. Alice's generator voltages are unknown to her. Eve uses the same protocol as mentioned in the bilateral case (see Section~\ref{bilateral}) to determine $R_{\mathrm{B}}$, but because Alice’s generator voltages are unknown to her, she cannot use Eq.~\eqref{Iw} to solve for $R_{\mathrm{A}}$. Instead, she uses the KLJN protocol as Bob does: use the entire bit exchange period to evaluate the measured mean-squared voltage on the wire. From that value, by using Eq.~\eqref{meansquare}, she evaluates the parallel resultant $R_{\mathrm{P}}$ of the resistances of Alice and Bob. From $R_{\mathrm{P}}$ and $R_{\mathrm{B}}$, she can calculate $R_{\mathrm{A}}$. This method can still be applied in case Eve is not sure of her result from the bilateral case (see Section~\ref{bilateral}).

\subsection{Timing}
\label{timing}
In each attack, Eve may or may not know which noise belongs to which resistor, or the noises may provide a voltage-to-current ratio that results in either $R_{\mathrm{H}}$ or $R_{\mathrm{L}}$. In these scenarios, there will be a negligible waiting/verification (no-response) time before Eve can differentiate between the noises. The probability of the two independent noises being equal at any given point is

\begin{equation}
p_{\mathrm{0}}=\frac{1}{2^\Delta},\label{p0}
\end{equation}

\noindent where $\Delta$ is the number of resolution bits.

We can consider the event that the noises run identically for $n$ subsequent steps to be a geometric distribution, with a probability of

\begin{equation}
p=p_0^n,\label{p1}
\end{equation}

\noindent where $n=t/\tau$ and $\tau$ is the autocorrelation time, given by the Nyquist Sampling Theorem

\begin{equation}
\tau\approx\frac{1}{2\Delta f_{\mathrm{B}}}.\label{tau}
\end{equation}

\noindent The approximation sign is due to the quantized nature of the noises, as they are constant throughout the bit exchange periods.

While such an identical match between the two noises is taking place, Eve cannot distinguish between the two noises, thus the actual resistance situation (see Fig.~\ref{threelevels}) remains secure. However, the exponential decay in Eq.~\eqref{p1} yields an efficient cracking scheme of the secure key bit value within a short amount of time. In accordance with Eq.~\eqref{p1}, the probability of the two independent seeds running identically is

\begin{equation}
p\approx p_0^{t/\tau}\approx\left(\frac{1}{2^\Delta}\right)^{t/\tau}.\label{p}
\end{equation}

\section{Conclusion}
\label{conclusion}
Secure key exchange protocols utilize random numbers, and compromised random numbers lead to information leak. So far, it had been unknown how Eve can utilize compromised random number generators to attack the KLJN protocol. To demonstrate how compromised RNGs can be utilized by Eve, we have introduced two simple attacks on the KLJN scheme.

We showed that if Eve knows the root of both Alice’s and Bob’s RNGs, that is, when she exactly knows the random numbers, she can use Ohm’s Law to crack the bit exchange. Eve can extract the bit very quickly, and she will learn the exchanged bit faster than Alice and Bob who know only their own random numbers.

We have also shown that if Eve knows the seed of only Bob’s RNG, she can still use Ohm’s Law to crack the secure bit. However, she is required to utilize the whole bit exchange period.

No statistical evaluation is needed, except for in the rarely-occurring event that Eve does not know which RNG belongs to which resistor, which will render in a waiting/verification (no-response) time that has a negligible effect on Eve’s cracking scheme.

It is important to note that:
\begin{itemize}
\item To utilize these attacks, we implicitly used Kerckhoffs’s principle/Shannon's maxim \cite{Kerckhoffs}, which means Eve knows all the fine details of the protocol, including how the seeds are utilized and the RNG outputs timed.
\item This demonstration was done assuming an ideal KLJN scheme. Future work would involve a practical implementation with a cable simulator and related delays and transients.
\item A deterministic knowledge of the random number(s) by Eve is a strong security vulnerability. However, it is an illustrative way how such attacks can be developed.
\item Open problems are new attack schemes where Eve's knowledge of the RNGs is only statistical \cite{RNG}.
\end{itemize}



==> data/section1b.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Fall 2016.  
%
%
%  Author: Sean Zachary Roberson
%  Version 3.17.09
%  Last Updated: 9/21/2017
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                           SECTION I
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\pagestyle{plain} % No headers, just page numbers
\pagenumbering{arabic} % Arabic numerals
\setcounter{page}{1}


\chapter{\uppercase {Random Number Generator Attack against the Kirchhoff-Law-Johnson-Noise Secure Key Exchanger}}

\section{Background}

\subsection{Random Number Generator Attacks}
\label{RNG}

There are two classes of practical random number generators: true (physical) and computational. The nature of computational RNGs is that they collect randomness from various low-entropy input streams and try to generate outputs that are in practice indistinguishable from truly random streams \cite{RNG1,RNG2,RNG3,RNG4,RNG5,RNG6}. The randomness of an RNG relies on the uncertainty of the random seed, or initialization vector, and a long sequence with uniform distribution. The moment an adversary learns the seed, the outputs are known, and the RNG is compromised.

Various RNG attacks exist against conditional secure communications \cite{RNG1,RNG2,RNG3,RNG4,RNG5,RNG6}. Unconditional secure communications also require true random numbers for perfect security and that is also true for the noises of Alice and Bob, and for the randomness of their switch driving. Yet it is unclear how Eve can utilize compromised RNGs to attack the KLJN scheme. Here we demonstrate with simple attack examples that compromised noises lead to information leak. 

The rest of this chapter is organized as follows. Section~\ref{RNGexperiment} describes the new attack protocol, Section~\ref{RNGresults} demonstrates the results, and Section~\ref{RNGconclusion} closes this paper.

\section{Attack Methodology}
\label{RNGexperiment}

Two situations are introduced where Eve can use compromised RNGs to crack the KLJN scheme: one where Eve knows the seed of both Alice’s and Bob’s generators (bilateral parameter knowledge), and another where Eve knows the seed of only Alice’s generator (unilateral parameter knowledge).

\subsection{Bilateral Parameter Knowledge}
\label{bilateral}
Eve knows the seed of both Alice’s and Bob’s RNGs, thus she knows the instantaneous amplitudes of the noise voltage generators for each of their resistors (see Fig.~\ref{figKLJN}). With $U_{\mathrm{H,A}}(t)$, $U_{\mathrm{L,A}}(t)$, $U_{\mathrm{H,B}}(t)$, and $U_{\mathrm{L,B}}(t)$ known, Eve uses \eqref{Uw} and \eqref{Iw} to come up with the four possible waveforms for $U_{\mathrm{w}}(t)$ and $I_{\mathrm{w}}(t)$ and therefore the four possible waveforms for the instantaneous power flow from Alice to Bob, given by

\begin{equation}
P_\mathrm{w}(t)=U_\mathrm{w}(t)I_\mathrm{w}(t).\label{Pw}
\end{equation}

\noindent Eve measures $U_{\mathrm{w}}(t)$ and $I_{\mathrm{w}}(t)$ and determines the actual $P_{\mathrm{w}}(t)$, which will be identical to one of her four hypothetical waveforms.

Note, the protocol shown above can be simplified to the extreme: Eve's instruments may have just one bit resolution, which is suitable to determine solely the instantaneous direction of the power flow.

\subsection{Unilateral Parameter Knowledge}
\label{unilateral}
Eve knows the seed of Alice’s generator RNG. Thus she knows merely the noise generator outputs of Alice’s resistors, $U_{\mathrm{L,A}}(t)$ and $U_{\mathrm{H,A}}(t)$. Bob’s generator voltages are unknown by her. Eve measures the wire voltage $U_{\mathrm{w}}(t)$ and wire current $I_{\mathrm{w}}(t)$. Then she calculates the hypothetical voltage drops on Alice's possible choice of resistances $R_{\mathrm{H}}$ and $R_{\mathrm{L}}$. With these data, she tests two hypotheses:

\noindent\begin{description}%[leftmargin=!,labelwidth=\widthof{The longest label}]
\item [Hypothesis (i):] Alice has chosen $R_{\textrm{L}}$.
\item [Hypothesis (ii):] Alice has chosen $R_{\textrm{H}}$.
\end{description}

With Hypothesis (i), Eve takes the sum

\begin{equation}
U_{\mathrm{A}}(t)=U_{\mathrm{w}}(t)+I_{\mathrm{w}}(t)R_{\mathrm{L}}.\label{UA}
\end{equation}

\noindent To test Hypothesis (i) she compares the $U_{\mathrm{A}}(t)$ determined by \eqref{UA} to $U_{\mathrm{L,A}}(t)$. If they are identical then hypothesis (i) is correct, otherwise hypothesis (ii) is valid.

Finally, Eve evaluates the measured mean-square voltage on the wire over the bit exchange period. From that value, by using \eqref{meansquare}, she evaluates the parallel resultant $R_{\mathrm{P}}$ of the resistances of Alice and Bob. From $R_{\mathrm{P}}$ and $R_{\mathrm{A}}$, she calculates $R_{\mathrm{B}}$, thus she has cracked the KLJN scheme.

\section{Demonstration}
\label{RNGresults}

\subsection{Johnson Noise Emulation}

First, we generated Gaussian band-limited white noise (GBLWN). Precautions were used to avoid aliasing errors, improve Gaussianity and reduce bias:

\begin{enumerate}[label=(\roman*)]
\item At first, using the MATLAB randn() function, 2\textsuperscript{24} or 16,777,216 Gaussian random numbers were generated.

\item This process was repeated 10 times to generate 10 independent raw noise series, and then an ensemble average was taken out of those 10 series to create one single noise time function with improved Gaussianity and decreased short-term bias.

\item Then this time series was converted to the frequency domain by Fast Fourier Transformation (FFT). To get rid of any aliasing error, we opened the real and imaginary portions of the FFT spectrum and doubled their frequency bandwidths by zero padding.

\item Finally, we performed an inverse FFT (IFFT) of the zero-padded spectrum to get the time function of the anti-aliased noise.
\end{enumerate}

\noindent The real portion of the IFFT result is the band-limited, anti-aliased noise with improved Gaussianity and decreased bias.

The histogram and probability plot for the generated noise are shown in Figs.~\ref{hist_noise} and \ref{probplot_noise}, respectively, showing that the noise is Gaussian. Fig.~\ref{PSD_noise} demonstrates that the noise has band-limited, white power density spectrum and it is anti-aliased.

\begin{figure}[H]
\centering
	\includegraphics[width=4.25in]{hist_noise.pdf}
\caption{Histogram of the noise. A mean of zero and a standard deviation of 1 indicates a standard normal distribution.\label{hist_noise}}
\end{figure}

\begin{figure}[H]
\centering
	\includegraphics[width=4.25in]{probplot_noise.pdf}
\caption{Normal-probability plot of the noise. A straight line indicates a pure Gaussian distribution.\label{probplot_noise}}
\end{figure}

\begin{figure}[H]
\centering
	\includegraphics[width=4.25in]{PSD_noise.pdf}
\caption{Power spectral density of the noise. The bandwidth of the noise is 500 Hz, see \eqref{meansquare}.\label{PSD_noise}}
\end{figure}

The final step was to convert this normalized Gaussian noise to Johnson noise of physical values. Two separate independent noise files were created, by using the methods described above. A thousand points were used in this simulation. Their effective (RMS) values were scaled by the Johnson formula \eqref{meansquare} to the values relevant for the actual $T_\mathrm{eff}$, $R_\mathrm{L}$, $R_\mathrm{H}$, and $\Delta$$f_\mathrm{B}$. We chose $T_\mathrm{eff}$=10\textsuperscript{18} K, $R_\mathrm{L}$=10 k$\Omega$, $R_\mathrm{H}$=100 k$\Omega$, and $\Delta$$f_\mathrm{B}$=500 Hz. The histogram, probability plot, and power spectral density for the Johnson noise of $U_\mathrm{H,A}(t)$, $U_\mathrm{L,A}(t)$, $U_\mathrm{H,B}(t)$, and $U_\mathrm{L,B}(t)$, where $U_\mathrm{H,A}(t)$ is the noise voltage of Alice’s $R_\mathrm{H}$, $U_\mathrm{L,A}(t)$ is the noise voltage of Alice’s $R_\mathrm{L}$, $U_\mathrm{H,B}(t)$ is the noise voltage of Bob’s $R_\mathrm{H}$, and $U_\mathrm{L,B}(t)$ is the noise voltage of Bob’s $R_\mathrm{L}$ (see Fig.~\ref{figKLJN}), are shown in Figs.~\ref{hist}, \ref{probplot}, and \ref{PSD}, respectively.

\begin{figure}[H]
\centering
	\includegraphics[width=4.25in]{hist.pdf}
\caption{Histogram of the Johnson noise of $U_\mathrm{H,A}(t)$, $U_\mathrm{L,A}(t)$, $U_\mathrm{H,B}(t)$, and $U_\mathrm{L,B}(t)$, where $U_\mathrm{H,A}(t)$ is the noise voltage of Alice’s $R_\mathrm{H}$, $U_\mathrm{L,A}(t)$ is the noise voltage of Alice’s $R_\mathrm{L}$, $U_\mathrm{H,B}(t)$ is the noise voltage of Bob’s $R_\mathrm{H}$, and $U_\mathrm{L,B}(t)$ is the noise voltage of Bob’s $R_\mathrm{L}$ (see Fig.~\ref{figKLJN}). The blue histograms represent the occurrences of the noise voltages over time, and the yellow histograms represent the occurrences of the noise voltages sampled 1000 times at a specific time point. The green area represents the overlap between the blue and yellow histograms. The red line represents the normal probability density function (PDF) for both histograms, serving to demonstrate that the noise voltages in all four cases ($HH$, $LL$, $HL$, and $LH$) are Gaussian and ergodic.\label{hist}}
\end{figure}

\begin{figure}[H]
\centering
	\includegraphics[width=4.25in]{probplot.pdf}
\caption{Normal-probability plot of the Johnson noise of $U_\mathrm{H,A}(t)$, $U_\mathrm{L,A}(t)$, $U_\mathrm{H,B}(t)$, and $U_\mathrm{L,B}(t)$. A straight line indicates a pure Gaussian distribution.\label{probplot}}
\end{figure}

\begin{figure}[H]
\centering
	\includegraphics[width=4.25in]{PSD_noise.pdf}
\caption{Power spectral density of the Johnson noise of of $U_\mathrm{H,A}(t)$, $U_\mathrm{L,A}(t)$, $U_\mathrm{H,B}(t)$, and $U_\mathrm{L,B}(t)$. The bandwidth of the noise is 500 Hz, see \eqref{meansquare}.\label{PSD}}
\end{figure}

From the Nyquist Sampling Theorem

\begin{equation}
\tau=\frac{1}{2\Delta f_\mathrm{B}}\label{Nyquist}
\end{equation}

\noindent where $\tau$ represents the time step, a $\Delta$$f_\mathrm{B}$ of 500 Hz renders a time step of 10\textsuperscript{-3} seconds. Because this is ideal band-limited white noise, the Nyquist samples are statistically independent.

\subsection{Attack Demonstration when Eve Knows Both Noises}
\label{bidem}
At the bilateral parameter knowledge (see Section~\ref{bilateral}), a realization of the noise amplitudes over 100 milliseconds is displayed in Fig.~\ref{allvoltages}.

\begin{figure}[ht!]
\centering
	\includegraphics[width=4.25in]{allvoltages.pdf}
\caption{A realization of $U_\mathrm{H,A}(t)$, $U_\mathrm{L,A}(t)$, $U_\mathrm{H,B}(t)$, and $U_\mathrm{L,B}(t)$ (see Fig.~\ref{figKLJN}) displayed over 100 milliseconds. $U_\mathrm{H,A}(t)$ is the noise voltage of Alice’s $R_\mathrm{H}$, $U_\mathrm{L,A}(t)$ is the noise voltage of Alice’s $R_\mathrm{L}$, $U_\mathrm{H,B}(t)$ is the noise voltage of Bob’s $R_\mathrm{H}$, and $U_\mathrm{L,B}(t)$ is the noise voltage of Bob’s $R_\mathrm{L}$. Each time step is one millisecond.\label{allvoltages}}
\end{figure}

Fig.~\ref{1beve} shows the hypothetical power flow waveforms generated by Eve (top four graphs). The single-bit plot of her measurement of the actual power flow $P_\mathrm{w}(t)$ is shown by the bottom graph. If the power is delivered from Alice to Bob, the single-bit value is +1, while in the opposite case the result is -1. The orange dashed lines in the upper plots indicate the power flow in the 1-bit resolution limit. At the present situation, Eve’s measured single-bit data are identical to the dashed lines in the $LH$ scenario only, thus Eve decides that the $LH$ is the secure resistance situation.

\begin{figure}[ht!]
\centering
	\includegraphics[width=4.25in]{1beve.pdf}
\caption{The hypothetical and their 1-bit limit waveforms for $P_\mathrm{w}(t)$ generated by Eve. $P_\mathrm{HH}(t)$ is the hypothetical power flow in the $HH$ case, $P_\mathrm{LL}(t)$ is the hypothetical power flow in the $LL$ case, $P_\mathrm{HL}(t)$ is the hypothetical power flow in the $HL$ case, and $P_\mathrm{LH}(t)$ is the hypothetical power flow in the $LH$ case. $P_\mathrm{w}(t)$ is the single-bit measurement of the actual power flow.\label{1beve}}
\end{figure}

However, similarly to the case of string verification with noise-based logic \cite{NBL}, two independent random bit sequences, such as two different binary sequences in Fig.~\ref{1beve}, may run identically for $n$ subsequent steps with probability

\begin{equation}
P=\frac{1}{2^n}\label{probability}
\end{equation}

\noindent where the independence of the subsequent samples within a given binary sequence is also essential, and $n=t/\tau$.

While such an identical match between two of the 4 noises is taking place, Eve cannot decide which one of the hypothetical sequences is valid thus the actual resistor situation (see Fig.~\ref{threelevels}) remains secure. However, the exponential decay of the probability of the duration of this phenomenon \ref{probability} yields an efficient cracking of the secure key bit value within a short time. In accordance with \eqref{probability}, the probability of two independent ones of our binary sequences (Fig.~\ref{1beve}) running identically is

\begin{equation}
P(t)\approx\frac{1}{2^{t/\tau}}=\frac{1}{2^{1000t}}\label{poft}
\end{equation}

\noindent The approximation sign is due to the quantized nature of $P(t)$ because it is staying constant during the bit exchange periods.

This simulation was run 1000 times. Fig.~\ref{log_securecases} shows the probability that the exchange of the current key bit is still secure. Fig.~\ref{log_crack} shows the probability that Eve has already cracked the bit. The red lines follow the scaling given by \ref{poft}.

\begin{figure}[H]
\centering
\subfloat[]{
	\label{log_securecases}
	\includegraphics[width=2.12in]{CorrectguessvsBEP.pdf} } 
\subfloat[]{
	\label{log_crack}
	\includegraphics[width=2.12in]{CorrectguessvsBEPcomp.pdf} } 
\caption{Probabilities during the attack with single-bit resolution of Eve's measurements. (a) Probability that the exchange of the current key bit is still secure; (b) and probability that Eve has already cracked it. The histograms represent the simulation results, and the red lines represent the scaling given by \ref{poft}.}
\end{figure}

\subsection{Attack Demonstration when Eve Knows Unly One of the Sources}
\label{unidem}
At the unilateral parameter knowledge (see Section~\ref{unilateral}), Eve knows the seed of Alice’s RNG, while the seed of Bob’s RNG is unknown by her. Thus we suppose she knows $U_\mathrm{A}(t)$ (like at the bilateral case) but not $U_\mathrm{B}(t)$. A realization of the wire voltage and current, $U_\mathrm{w}(t)$ and $I_\mathrm{w}(t)$, under the $LH$ condition over 100 milliseconds is displayed in Fig.~\ref{Eve_wire_data}. Fig.~\ref{Possible_voltagedrops} shows the hypothetical noise voltages generated by Eve's simulations across $R_\mathrm{L}$ and $R_\mathrm{H}$ (see \ref{UA}).

\begin{figure}[H]
\centering
	\includegraphics[width=4.25in]{Eve_wire_data.pdf}
\caption{A realization of $U_\mathrm{w}(t)$ and $I_\mathrm{w}(t)$ (see Fig.~\ref{figKLJN}) displayed over 100 milliseconds. Eve measures and records these data.\label{Eve_wire_data}}
\end{figure}

\begin{figure}[H]
\centering
	\includegraphics[width=4.25in]{Possible_voltagedrops.pdf}
\caption{Hypothetical noise voltage drops across $R_\mathrm{L}$ and $R_\mathrm{H}$ by Eve's current measurements and Ohm's law. These results are used in \eqref{UA} to calculate the hypothetical waveforms for $U_\mathrm{L,A}(t)$ and $U_\mathrm{H,A}(t)$.\label{Possible_voltagedrops}}
\end{figure}

Fig.~\ref{Evecalc_vs_UA} shows Eve’s known $U_\mathrm{A}(t)$ in comparison with her hypothetical waveforms (see \eqref{UA}) for $U_\mathrm{L,A}(t)$ and $U_\mathrm{H,A}(t)$. In this case, the waveform for $U_\mathrm{A}(t)$ is identical to that of $U_\mathrm{L,A}(t)$, thus Eve decides that Alice has chosen $R_\mathrm{L}$. A correlation plot is also shown in Fig.~\ref{corr}. A one-to-one correlation between Eve's known $U_\mathrm{A}(t)$ and the hypothetical waveform for $U_\mathrm{L,A}(t)$ indicates that Alice has chosen $R_\mathrm{L}$.

\begin{figure}[H]
\centering
	\includegraphics[width=4.25in]{Evecalc_vs_UA.pdf}
\caption{Eve’s known $U_\mathrm{A}(t)$ and the hypothetical waveforms (see \ref{UA}) for $U_\mathrm{H,A}(t)$ and $U_\mathrm{L,A}(t)$.\label{Evecalc_vs_UA}}
\end{figure}

\begin{figure}[H]
\centering
	\includegraphics[width=4.25in]{corr_RL.pdf}
\caption{Correlation between Eve's known $U_\mathrm{A}(t)$ and the hypothetical waveforms (see \ref{UA}) for $U_\mathrm{H,A}(t)$ and $U_\mathrm{L,A}(t)$.\label{corr}}
\end{figure}

Finally, Eve evaluates the measured mean-square voltage on the wire over the bit exchange period, shown in Fig.~\ref{u2}. From that value, by using \eqref{meansquare}, she evaluates the parallel resultant $R_\mathrm{P}$ of the resistances of Alice and Bob. From $R_\mathrm{P}$ and $R_\mathrm{A}$, she can calculate $R_\mathrm{B}$. In this particular case, Bob has chosen $R_\mathrm{H}$, thus Eve has cracked the $LH$ situation and the related secure bit value.

\begin{figure}[H]
\centering
	\includegraphics[width=4.25in]{u2.pdf}
\caption{The hypothetical and measured mean-square voltage generated by Eve. $U_\mathrm{HH,eff}^2$ is the hypothetical mean-square voltage in the $HH$ case, $U_\mathrm{LL,eff}^2$ is the hypothetical mean-square voltage in the $LL$ case, $U_\mathrm{HL,eff}^2$ is the hypothetical mean-square voltage in the $HL$ case, and $U_\mathrm{LH,eff}^2$ is the hypothetical mean-square voltage in the $LH$ case. $U_\mathrm{w,eff}^2$ is the measurement of the actual mean-square voltage.\label{u2}}
\end{figure}

\section{Conclusion}
\label{conclusion}
Secure key exchange protocols utilize random numbers and compromised random numbers lead to information leak. So far, it had been unknown how Eve can utilize compromised random number
generators to attack the KLJN protocol.

To demonstrate how compromised RNGs can be utilized by Eve, we have introduced two simple attacks on the KLJN scheme.

In Section~\ref{bidem} we showed that if Eve knows the seed of both Alice's and Bob's RNGs, that is, when she exactly knows the random numbers, she can crack the bit exchange even if her measurements have only one bit of resolution. The situation is similar to string verification in the noise-based logic systems. The cracking of the exchanged bit is exponentially fast; Eve can extract the bit within a fraction of the bit exchange period. Thus Eve will learn the exchanged bit faster than Alice and Bob who know only their own random numbers.

We have also shown in Section~\ref{unidem} that if Eve knows the seed of only Alice’s RNG, she can still crack the secure bit however she is required to utilize the whole bit exchange period.

It is important to note that:
\begin{itemize}
\item This demonstration was done assuming an ideal KLJN scheme. Future work would involve a practical
implementation with a cable simulator and related delays and transients.
\item A deterministic knowledge of the random number(s) by Eve is a strong security vulnerability, however
it is an illiustrative way how such attacks can eb developed;
\item Open problems are new attack schemes where Eve's knowledge is only statistical.
\end{itemize}




